Let the CAT out of the bag: Contrastive Attributed explanations for Text

Contrastive explanations for understanding the behavior of black box models has gained a lot of attention recently as they provide potential for recourse. In this paper, we propose a method Contrastive Attributed explanations for Text (CAT) which provides contrastive explanations for natural language text data with a novel twist as we build and exploit attribute classifiers leading to more semantically meaningful explanations. To ensure that our contrastive generated text has the fewest possible edits with respect to the original text, while also being fluent and close to a human generated contrastive, we resort to a minimal perturbation approach regularized using a BERT language model and attribute classifiers trained on available attributes. We show through qualitative examples and a user study that our method not only conveys more insight because of these attributes, but also leads to better quality (contrastive) text. Quantitatively, we show that our method outperforms other state-of-the-art methods across four data sets on four benchmark metrics.

==> Contrastive Attributed Text Explanation/abs.tex <==
%!TEX root = main_v0.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 							Abstract
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
% Despite the tremendous success of neural dialogue models in recent years, it suffers a lack of relevance, diversity, and some times coherence in generated responses. Lately, transformer-based models, such as GPT-2, have revolutionized the landscape of dialogue generation by capturing the long-range structures through language modeling. Though these models have exhibited excellent language coherence, they often lack relevance and terms when used for domain-specific response generation. In this paper, we present DSRNet (Domain Specific Response Network), a transformer-based model for dialogue response generation by reinforcing domain-specific attributes. In particular, we extract meta attributes from context and infuse them with the context utterances for better attention over domain-specific key terms and relevance. We study  the use of DSRNet in a multi-turn multi-locuter environment for domain-specific response generation. In our experiments, we evaluate DSRNet on Ubuntu-Dialogue dataset, which are mainly composed of various technical domain related dialogues for IT domain issue resolutions and on CamRest dataset, which contains restaurant domain conversation. Trained with maximum likelihood objective, our model shows significant improvement over the state-of-the-art for multi-turn dialogue systems supported by better BLEU and semantic similarity (BertScore) scores. Besides, we also observe that the responses produced by our model carry higher relevance due to the presence of domain-specific key attributes that exhibit better overlap with the attributes of the context. Our analysis shows that the performance improvement is mostly due to the infusion of key terms along with dialogues which result in better attention over domain-relevant terms. Other contributing factors include joint modeling of dialogue context with the domain-specific meta attributes and topics.

Contrastive explanations have gained a lot of attention recently as they provide potential for recourse. In this paper, we propose a method Contrastive Attributions for Text (CAT) which provides contrastive explanations for natural language text data with a novel twist as we build and exploit attribute classifiers leading to more semantically meaningful explanations. We show through qualitative examples and a user study that our method not only conveys more insight because of these attributes, but also leads to better quality (contrastive) sentences. Moreover, quantitatively we show that our method is more efficient than other state-of-the-art methods with it also scoring higher on benchmark metrics such as COLA.

Contrastive explanations have gained a lot of attention recently as they provide potential for recourse. In this paper, we propose a method Contrastive Attributions for Text (CAT) which provides contrastive explanations for natural language text data with a novel twist as we build and exploit attribute classifiers leading to more semantically meaningful explanations. %Our model provides attributions edits for a contrastive explanation. 
%To ensure minimal edits while generating contrastive explanations which are fluent and consistent with human contrastives, we resort to a targeted perturbation through BERT model. 
To ensure least edits while generating contrastive explanations while also fluent and consistent with human generated contrastives, we resort to a minimal perturbation approach through BERT model.
%To produce contrastive explanations with that are not only 
%We propose to a targeted perturbation through based approach to ensure 
%To ensure minimal changes and fluent sentence generation for contrastive explanation, we resort to a targeted perturbation using BERT based model. 
We show through qualitative examples and a user study that our method not only conveys more insight because of these attributes, but also leads to better quality (contrastive) sentences. Moreover, we show that our method is effective and more efficient than other relevant state-of-the-art methods through both quantitative and qualitative analysis.
%Moreover, quantitatively we show that our method is more efficient than other state-of-the-art methods with it also scoring higher on benchmark metrics such as COLA.
\end{abstract}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% to add and emphasize 
% meta context

==> Contrastive Attributed Text Explanation/appen.tex <==
\appendix
\section{Appendix}
% \twocolumn[\centering\Large\bfseries Let the CAT out of the bag: \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext\\
% (Supplement) \par \medskip]

% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on four metrics: 1) \textbf{Flip} rate, ii) \textbf{Dist}(distance), iii) \textbf{Fluency}, iv) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev) for all the metrics for CAT.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|cccc|cccc}
% \multicolumn{9}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{4}{c|}{AgNews} &
%       \multicolumn{4}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Flip & Dist & Cont & Fluency &
%       Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.164 $  &$0.110 $  & $0.286$ &$0$  &$0.140$  &$0.105$  &$0.467$  \\
%       std. dev.(CAT) &$0$  &$0.098 $  &$0.084 $  & $0.105$ &$0$  &$0.100$  &$0.076$  &$0.134$  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{4}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       &Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.132 $  &$0.115 $  & $0.344$ \\
%       std. dev.(CAT) & $0$  &$0.059 $  &$0.069 $  & $0.064$ \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}

\subsection{Quantitative Evaluation Statistics}
Table \ref{tab:quant} shows the performance evaluation of our proposed approach, CAT, on five different datasets. It was noted that CAT outperformed GYC over AgNews, Yelp and Dbpedia by statistically significant margins. We verify this statement in Table \ref{tab:quant_stat} where we report pairwise t-tests comparing the means for CAT and GYC and standard deviation of CAT for each metric and dataset. The improvement of CAT over GYC is observed to be statistically significant across all metrics. We do not report additional statistics for the flip rate metric as CAT always produces a contrastive sentence with a flipped class label unlike GYC which sometimes fails to flip.

\begin{table*}[h]
 \centering
\caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
}
 \label{tab:quant_stat}
\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.164   &0.110   &0.286  &0.140  &0.105  &0.467  \\
      std. dev. (CAT)   &\textbf{0.098}  &\textbf{0.084} &\textbf{0.105 } &\textbf{0.100} &\textbf{0.076} &\textbf{0.134}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|cccccccc}
\multicolumn{4}{c}{}\\
\multirow{3}{*}{Stat} &
    %  \multicolumn{4}{c|}{NLI} &
      \multicolumn{3}{c}{Dbpedia} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
    %   & Flip & Dist & Cont & Fluency 
       & Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
      p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
      \midrule
      std. dev.(GYC)  &0.132   &0.115   &0.344 \\
      std. dev.(CAT)   &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} \\
    %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
      \bottomrule
  \end{tabular}
  
% \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Method} &
%       \multicolumn{4}{c}{Hate Speech} \\
%       & Flip & Dist & Cont & Fluency\\
%         \midrule
%       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
%       \bottomrule
%   \end{tabular}
  \label{tab:quant_stat}
\end{table*}

\begin{table}[htbp]
\centering
\small
\caption{Extra contrastive explanation examples from five datasets: AgNews, Hate Speech, NLI, DBPedia, and Yelp.}
\label{tab:extra_examples}
\begin{tabular}{|p{7cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Input/CAT}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Attribute Changes}}}  & \multicolumn{1}{c|}{\textbf{Input}} & \multicolumn{1}{c|}{\textbf{Contrast}}
& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}}\\
   &  & \multicolumn{1}{c|}{\textbf{Pred}}  &\multicolumn{1}{c|}{\textbf{Pred}}&  \\ \hline

\st{Oil} \textcolor{red}{Winds} Up from 7-Week Lows on U.S. Weather & \multicolumn{1}{c|}{+travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{world} & AgNews \\ \hline

New Hummer Is Smaller, Cheaper and Less \st{Gas} \textcolor{red}{cpu} Hungry & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -travel, \\-space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ 
\hline

\multirow{2}{*}{Perfect start for France in \st{Federation} \textcolor{red}{Microsoft} Cup} & \multirow{2}{*}{\shortstack{+cryptography, -motorcycles, \\-hockey, -space, -politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey}& \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\st{Kuwait} \textcolor{red}{Source}: Fundamentalists Recruiting Teens (AP) &  \multicolumn{1}{c|}{+guns, religion, -mideast}& \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\multirow{2}{*}{Harry \st{in nightclub} \textcolor{red}{inflight} scuffle}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+sports, +space, -religion, \\-cryptography, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

I thought you \textcolor{red}{ladies} were leaving the country you washed up \$\$\$\$ \$\$\$\$? & \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -cryptography}}& \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

Such crimes must attract severest punishment,say Min Jail term of 25Y. If they r \st{illegal} \st{migrants} \textcolor{red}{convicted}, force them to leave the Country immediately& \multicolumn{1}{c|}{\multirow{3}{*}{+atheism, -politics}} & \multicolumn{1}{c|}{\multirow{3}{*}{hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{Hate}} \\ \hline

\multirow{2}{*}{\st{@brianstelter} \textcolor{red}{she} is a complete \st{joke} \textcolor{red}{\$\$\$\$} ! if you see...}& 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +cryptography, \\-sports, -politics}} }& \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Do \st{you} \textcolor{red}{chicks} ever \st{rap} \textcolor{red}{talk} in your whitest voice possible or is that just me?& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+parenting, +atheism, +politics \\-world, -sports, -arts}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

\st{There's} \textcolor{red}{Women} \textcolor{red}{get} no greater satisfaction than knowing you did it yourself' -me when someone asks me ... & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +entertainment, \\ +religion, -sports}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

Five soldiers hold and aim their \st{weapons} \textcolor{red}{blades}. $<$/s$>$ The soldiers are \st{eating} \textcolor{red}{armed}.
& \multicolumn{1}{c|}{\multirow{2}{*}{-guns}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Skateboarder jumps of off dumpster. $<$/s$>$ a \st{bike} \textcolor{red}{young} rider in a race&
 \multicolumn{1}{c|}{\multirow{2}{*}{+world}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Two people walking down a dirt trail with backpacks on looking at \st{items} \textcolor{red}{map} they are carrying. $<$/s$>$ One is holding a map.
& \multicolumn{1}{c|}{\multirow{3}{*}{+space, -motorcyles, -electronics}}& \multicolumn{1}{c|}{\multirow{3}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

A brown and black dog is jumping to catch a red ball. $<$/s$>$ Two dogs are
\textcolor{red}{not} playing catch with their owner.
& \multicolumn{1}{c|}{\multirow{2}{*}{-arts}}& \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

A girl is standing in a field pushing up her hat with one finger and her hand is
covering most of her face. $<$/s$>$ A \st{girl} \textcolor{red}{boy} covers her face. 
& \multicolumn{1}{c|}{\multirow{3}{*}{+parenting, -medicine}}& \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

Channel Chaos is a 1985 Australian \st{film} \textcolor{red}{production} set at a TV station & \multicolumn{1}{c|}{\multirow{2}{*}{+electronics, -travel, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{film}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

\multirow{2}{*}{Dinik is a \st{village} \textcolor{red}{lake} in Croatia}
& \multicolumn{1}{c|}{\multirow{2}{*}{+medicine, +space, -mideast}}& \multicolumn{1}{c|}{\multirow{2}{*}{village}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{natural\\place}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

\multirow{2}{*}{Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}}
& \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{plant}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{written\\work}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

ACTION is a bus service \st{operator} \textcolor{red}{based} in Canberra Australia
& \multicolumn{1}{c|}{\multirow{2}{*}{+autos, -electronics}}& \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{transport\\-ation}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

Jagjaguwar is an indie rock record \st{label} \textcolor{red}{musician} based in Bloomington Indiana 
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+space, +politics, -world \\-forsale, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{artist}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

he \st{really} \textcolor{red}{hardly} made our anniversary dinner entertaining memorable
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +sports, +cryptography \\-home\&living, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

they also have deep fried desserts if you're \st{brave} \textcolor{red}{poor} enough
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+medicine, -travel \\-religion, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

i \st{definitely} \textcolor{red}{never} will go back & \multicolumn{1}{|c|}{-entertainment} &\multicolumn{1}{c|}{positive}&\multicolumn{1}{c|}{negative}&\multicolumn{1}{c|}{Yelp} \\ \hline

\multirow{2}{*}{jesse is completely \st{rude} \textcolor{red}{perfect}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -entertainment, \\-medicine, -space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

\multirow{2}{*}{the pizza \st{sauce} \textcolor{red}{heaven} is also way too sweet} & 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +travel, +arts, +atheism \\+religion, -medicine, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline


\eat{
\multirow{2}{*}{Kazaa Owner Cheers \st{File} \textcolor{red}{Salary}-Swapping Decision (AP)} \quad\quad\quad\quad\quad\quad\quad\quad & \multirow{2}{*}{\shortstack{+forsale, +baseball, +hockey,\\ -arts, -windows, -cryptography}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \\
\hline

New Human Species \st{Discovered} \textcolor{red}{influenza} & +medicine, -cryptography & \multicolumn{1}{c|}{sci-tech} & \multicolumn{1}{c|}{world} \\ \hline

US shows flexibility on \st{Israeli} \textcolor{red}{virtual} settlements & +arts, +cryptography, -mideast & \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} \\ \hline


\eat{Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey} & \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{business} \\ \hline}

Pace of U.S. \st{Factory} \textcolor{red}{population} Growth Climbs in Dec & \multicolumn{1}{c|}{+politics, -money, -travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{sci-tech} \\ \hline

It may take 146 years for Nigeria to wipe out \st{corruption} \textcolor{red}{funds} from \st{its} \textcolor{red}{bank} system going by the latest report ...\eat{by Transparency International (TI) which gave the country the third position among the most corrupt countries of the world} & \multicolumn{1}{c|}{\multirow{2}{*}{+ money, - politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} \\ \hline
}
\end{tabular}
 \end{table}


\subsection{Additional Setup Details}
All experiments were run on NVIDIA V100 GPUs. Since no ground truth exists for our contrastive explanations, hyperparameters for CAT objective (given in Eq.\ref{eqn:main}) were tuned qualitatively by observation. It is important to consider that, in practice a user will only need to tune the hyperparameters once at the beginning and will then be able to generate explanations for an arbitrary number of instances from the dataset. Our tuning led to the following values which we used across datasets: We kept highest weights for $\lambda = 5.0$ to make sure that perturbed sentences have a label different from that of original sentence. We used mean of BERT logits of words inserted/replaced as a surrogate for $p_{LM}(x')$ with regularization parameter $\eta$ set to be $1.0$ and regularization parameter $\nu$ for Levenshtein distance set to $2.0$. $\beta$ was set to $3.0$. We used two values of $\tau$. For binary attribute classifiers from the Huffpost News dataset, we set $\tau = 0.3$, and for multiclass attribute classifiers trained on the 20 Newsgroup dataset, we set $\tau=0.05$. Attribute classifiers were trained with DistliBERT base for $10$ epochs using the Adam optimizer with a learning rate of $5\times 10^{-5}$, weight decay of $0.01$, and a batch size of $16$.

Of the five black box models experimented in the paper, models trained on NLI and the Hate Speech dataset were directly taken from the huggingface website. %Yelp, AgNews, and DBpedia were trained 
%\textcolor{blue}{Amar to add details of BoW models such as architecture, optimizer, learning rate etc.}
The black box models for AgNews, DBPedia and Yelp is composed of an EmbeddingBag layer followed by a linear layer, a ReLU and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss for 4, 14 and 2 classes for AgNews, DBPedia and Yelp, respectively. The model is trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$. 

 \subsection{Additional Information for User Study}
 Figure \ref{fig:userinstr} shows screenshots of the user study, including the instructions and example questions for \eat{the three} different methods discussed in the study. For the users the methods were named as Explainer A, B and C, where they correspond to GYC, CAT, and CAT-na respectively. Some users also left optional comments at the end of the user study which we list here:
\vspace{-1pt}
 \begin{itemize}
     \item ``I found the questions confusing... What is complete, sufficient and understandable explanation in a word change? Also, in each example, what was I supposed to guess, the category of the article or the possible prediction of the method? Are those things different?''
     \item ``Explainer A was pretty bad, explainer B was very good, and explainer C was reasonably good.''
     \item ``Explainer b was the best. The q\&a at the end of each page allows multiple choices per row, which is bad. Each question should remove the modified classification as an option (if the modified sentence is World, I shouldn't be allowed to choose World). Early on the survey should state clearly that there are only 4 categories (business/sci-tech/sports/world) which I didn't know right away, I expected each question have 4 different options, and knowing this might have helped me understand what we're doing here better. The opening text was very confusing.''
     \item ``I found B to be the best one.''
     \item ``nice survey''
 \end{itemize}

 \begin{figure*}[htbp]
 \centering
  \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/CAT_instr.png}
         \caption{}
     \end{subfigure}
      \begin{subfigure}[b]{0.49\textwidth}
        \centering
         \includegraphics[width=\textwidth]{figs/likert_ss.png}
         \caption{}
     \end{subfigure}\\%   %\vspace{0.2cm}
   \begin{subfigure}[b]{0.39\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/gyc_ss.png}
         \caption{}
     \end{subfigure}
   \hspace{0.1\textwidth}
   \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/cat_ss.png}
        \caption{}
     \end{subfigure}
   \caption{In (a) we show the instructions for the survey. In (b) we see the qualitative questions. In (c) and (d) we see the task oriented questions for GYC and CAT respectively.} 
 \label{fig:userinstr}
 %\vspace{-0.3cm}
 \end{figure*}

\subsection{Additional Qualitative Examples}
Table \ref{tab:extra_examples} offers at least five more examples of contrastive explanations from each dataset. Additional insight can be gained from the attributes; in the first row, adding travel-related text can flip the class from business to world, i.e., the article was predicted business because if it was more about travel it would have been predicted as world. This type of explanation adds extra intuition as opposed to only being given the replacement of words, ``oil" to ``winds" in this case. As can also been seen, insight is also a function of using attributes that have a relationship to the dataset and task. For example, attributes derived from news sources are often not helpful for explaining sentiment classifiers (e.g., Yelp) for which sentiment is often flipped by the negation of the text. This is to be expected; good explanations require good attributes.
 

==> Contrastive Attributed Text Explanation/approach.tex <==
%!TEX root = main.tex
We now describe our \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext  (\textbf{CAT}) method. Contrastive explanations, convey why the model classified a certain input instance to a class $p$, and not another class $q$. This is achieved by creating contrastive examples (also called contrasts) from input instance which get predicted as $q$. Contrastive examples are created by minimally perturbing the input such that the model prediction changes. In the case of text data, perturbations can be of three types: (1) inserting a new word, (2) replacing a word with another, and (3) deleting a word. In addition to keeping the number of such perturbations small, constrastive explainers also try to maintain grammatical correctness and fluency of the contrasts \cite{gyc, mice}. 

As an example, take the case of a black box model trained on the AG News dataset that predicts which category a certain news headline falls under. Given a headline, %\\
%\indent 
``\textit{Many technologies may be a waste of time and money, researcher says}" %\\
which is predicted as Sci-Tech, a contrastive explainer will try to explain why this headline wasn't predicted as, say, \textit{Business} by generating a contrastive example,%\\
%\indent 
``\textit{Many \st{technologies} \textcolor{red}{jobs} may be a waste of time and money, researcher says}" %\\
which is predicted as Business. Observe that a single word replacement achieves a prediction change. Such contrastive explanations can help users test the robustness of black box classification models.

We observed that even with constraints for minimal perturbation and fluency on a given black box model and an instance, there are multiple contrastive examples to choose from and, very often, many are less informative than others. For example, another possible contrast is, %\\
%\indent 
``\textit{Many technologies may be a waste of \st{time} \textcolor{red}{investment} and money , researcher says"} %\\
which also gets predicted as Business. However, this particular explanation is not as intuitive as the previous one as ``money" is a form of ``investment" and the nature of the sentence has not changed in an obvious sense with the word ``technologies" still present in the sentence. 

To alleviate this problem, we propose to construct and use a set of \textit{attribute classifiers}, where the attributes could be tags/subtopics relevant to the classification task 
obtained from the same or a related dataset used to build the original classifier. Attribute classifiers indicate the presence/absence of a certain subtopic in the text and confidence scores from these classifiers could be used as a regularization to create a contrast. We thus prefer contrasts which change attribute scores measurably as opposed to those contrasts which do not. However, at the same time, we want a minimal number of attribute scores to change so as to have crisp explanations. Hence, our regularization not only creates more intuitive contrasts, but also provides additional information to the user in terms of changed subtopics which, as confirmed through our user study in Section \ref{sec:human}, provide better understanding of the model behavior. The important steps in our method are depicted in Figure \ref{fig:cat}.

Formally, given an input text $x \in \mathcal{X}$, and a text classification model $f(\cdot)$ which predicts $y = f(x)\in \mathcal{Y}$, we aim to create a perturbed instance $x'$ such that the predictions $f(x) \neq f(x')$ and $x'$ is ``minimally" different from $x$. We use a set of $m$ attribute classifiers $\zeta_i: \mathcal{X} \rightarrow \mathbb{R} , \forall i \in \{1,\ldots,m\}$, which produce scores indicative of presence (higher scores) or absence (lower scores) of corresponding attributes in the text. We say that attribute $i$ is added to the perturbed sentence if $\zeta_i(x') - \zeta_i(x) > \tau$ and removed when $\zeta_i(x') - \zeta_i(x) < -\tau$, for a fixed $\tau > 0$. Word-level Levenshtein distance between original and perturbed instance $d_{Lev}(x',x)$, which is the minimum number of deletions, substitutions, or insertions required to transform $x$ to $x'$ is used to keep the perturbed instance close to the original. The naturalness (fluency) of a generated sentence $x'$ is quantified by the likelihood of sentence $x'$ as measured by the language model used for generation; we denote  this likelihood by $p_{\text{LM}}(x')$.
For a predicate $\phi$, we denote $\mathbbm{1}_\phi$ the indicator of $\phi$, which takes the value 1 if $\phi$ is true and $0$ otherwise. Given this setup, we propose to find contrastive examples by solving the following optimization problem:
\begin{align}
\label{eqn:main}
    \max_{x' \in \mathcal{X}}&~~~  ||\zeta(x') - \zeta(x)||_{\infty}-\beta\sum_{i} \mathbbm{1}_{|\zeta_i(x') - \zeta_i(x)|>\tau} \nonumber \\
    & ~~~+ \lambda \cdot \max_{j \in \mathcal{Y}\setminus y} \{~[f(x')]_j - [f(x)]_y~\} \nonumber \\
    & ~~~+ \eta \cdot p_{\text{LM}}(x') ~-~\nu \cdot d_{Lev}(x',x),
\end{align}
where $\zeta(x)$ is a vector such that $[\zeta(x)]_i=\zeta_i(x)$, $\beta, \lambda, \eta, \nu > 0$ are hyperparameters that trade-off different aspects, and $||\cdot||_{\infty}$ is the $l_{\infty}$ norm. The first term in the objective function encourages to pick an $x'$ where at least one attribute is either added/removed from $x$. The second term minimizes the number of such attributes for ease of interpretation. The third term is the contrastive score, which encourages the perturbed instance to be predicted different than the original instance. Fourth and fifth terms ensure that the contrast is fluent and close to the original instance, respectively.

The above objective function defines a controlled natural language generation problem. Earlier methods for controlled generation that shift the latent representation of a language model (such as GPT-2) \cite{gyc, pplm} have resulted in generated sentences being very different from the original sentence. We thus adopt a different strategy where we first take the original sentence and identify locations where substitutions/insertions need to be made using available feature attribution methods such as Integrated Gradients \cite{integrated_gradients}. %We then use an MLM pretrained language model \cite{transformer, bert} to do that. 
%This approach is similar to \cite{mask_infill}, but their system only work on changing sentiment of text. 
%We use feature-importance based explainability methods, Integrated Gradients (IG) \cite{integrated_gradients} to identify important words. 
These words are ordered by their attribution and greedily replaced with a \texttt{[MASK]} token. An MLM pre-trained BERT model \cite{transformer, bert} is then used to fill these masks. We take the top $k$ such replacements ranked by BERT likelihood. For insertions, a mask token is inserted to the right and left of important words in order to generate a set of perturbations similar to the input example. The attribute classifiers are applied to each generated candidate contrast, and the best $x'$ is selected as evaluated by Eq. \ref{eqn:main}. 

% \subsection{Text perturbation}
% How BERT is used to create perturbed sentences. How this choice makes whole optimization to a combinatorial one vs continuous. Arguments to back why this is better.


==> Contrastive Attributed Text Explanation/conc.tex <==
%!TEX root = main.tex

%%% 							Concluding Remarks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
In this paper, we proposed a contrastive explanation method, CAT, with a novel twist where we construct attribute classifiers from relevant subtopics available in the same or different dataset used to create the black box model, and leverage them to produce high quality contrasts. The attributes themselves provide additional semantically meaningful information that can help gain further insight into the behavior of the black box model. We have provided evidence for this through diverse qualitative examples on multiple datasets, a carefully conducted user study and through showcasing superior performance on four benchmark quantitative metrics. In the future, it would be interesting to test this method on other applications with the appropriate attribute classifiers.

==> Contrastive Attributed Text Explanation/exp.tex <==
%!TEX root = main.tex
%%% 						Experiments and Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Setup Details}
We use an MLM pre-trained BERT\footnote{https://huggingface.co/bert-base-uncased} from Huggingface \cite{huggingface} to generate text perturbations. For attributes, classes from the Huffpost News-Category \cite{news_category} and 20 Newsgroups \cite{kaggle20NewsGrp} datasets were used. The Huffpost dataset has 200K news headlines split into 41 classes. We merged similar classes and removed those which weren't a standard topic; 22 classes remained. The 20 Newsgroups dataset has 18000 newsgroup posts with 20 topic classes. Together, we obtained 42 attributes. For 22 classes from Huffpost, we trained 22 1-vs-all binary classifiers with a distilbert \cite{distilbert} base, so that the same sentence can have multiple classes. For 20 Newsgroups, we trained multiclass classifiers with a distilbert base on the other 20 classes. 
More details on setup details are provided in appendix.
% Please refer to the Supplement for more details such as hyperparameter settings for CAT.

We evaluate our explanation method on models trained on AgNews \cite{AgNews2015}, DBPedia \cite{Lehmann2015DBpediaA}, Yelp \cite{Shen2017}, NLI \cite{nli}, and Hate Speech \cite{hatespeech}. For an apples-to-apples comparison of our methods with GYC on AgNews, DBPedia and Yelp, we trained models with the same architecture as the ones in their work: that is an Embedding Bag layer followed by a linear layer. For NLI\footnote{https://huggingface.co/roberta-large-mnli} and Hate speech\footnote{https://huggingface.co/cardiffnlp/twitter-roberta-base-hate} we used a Roberta \cite{roberta} based model available in huggingface.

\subsection{Qualitative Evaluations}
% We evaluate our models on datasets from AgNews \cite{AgNews2015}, NLI \cite{nli}, %\cite{kaggleAGNews}
% Hate Speech\footnote{Hate Speech dataset is from SemEval 2019 task 5, available at {https://ash0904.github.io/IRE-Project-hatEval-2019}}, DBPedia \cite{Lehmann2015DBpediaA}, and Yelp \cite{Shen2017}.  %\cite{HateSpeech}
%All datasets are from different domains. In addition, we use 6-class version of $20$-Newsgroups topic classification dataset \cite{Lang1995,kaggle20NewsGrp} to train attribute classifiers. 

We now provide qualitative examples from three diverse datasets AgNews, NLI and Hate Speech. 
In appendix we provide additional examples from these and other datasets as well.
% More examples from these and other datasets are in the Supplement.

\noindent\textbf {AgNews}. The dataset is from a real-world news domain which contains short news headlines and bodies from four new categories - world, business, sports, and sci-tech. It contains ~30K training and ~1.9K test examples per class, comprising of ~128K samples. Our experiments focus on explanations for predicting the class from the headlines.

Table \ref{tab:agnews} shows results of applying CAT to five headlines in the AgNews dataset. 
% (more examples are in the Appendix). 
The first row explains that the headline is predicted as sci-tech because if the headline was more related to topics such as things for sale, baseball, hockey, and less about computer-related topics, it would have been predicted sports, which is achieved in the contrast by replace ``File" with ``Salary". It is important to consider the interaction of words; here, the black box model considers Kazaa a sports team because of the change. The second and third rows offer intuitive examples as to how the attribute changes relate to the contrasts. The insight is that we learn what topics the black box model finds most relevant to the prediction, as opposed to only knowing the single word and needing to figure out why that caused the change. \eat{The fourth row is not as intuitive, but digging deeper, we learned that replacing ``playoffs" by ``2019", ``2020", or ``2021" gave the same attribute changes and hence years are associated with the topic space, likely due to an interaction between the word ``resurface" and the years. Adding such a topic can still lead to an orthogonal contrast class such as business as the black box model associates ``Lowe" with the home improvement store after removing the word ``playoffs".} In the fourth row, adding politics and removing money leads to changing the input from business to sci-tech as ``factory growth" has more relationship to money while ``population growth" is related to politics. In the fifth row, we have the opposite as adding money and removing politics changes the input from world to business. This last example illustrates that, for longer text, single perturbations are often insufficient to flip the label and multiple changes are needed. These last two examples offer the insight that the classifier associates business with politics, which is not obvious a priori.

\noindent\textbf{Hate Speech}. The dataset is composed of hate speech tweets labelled as hate or non-hate. It contains about 8100 tweets for training and 900 tweets for testing out of which about 3700 hate tweets. The text in such tweets is much less structured and of much poorer grammar than the other datasets we experiment with. Nevertheless, CAT offers interesting insight as seen in Table \ref{tab:hate}. Note that we have hidden vulgar words (only for presentation purposes). 

The first two rows show contrasts that illustrate the black box model's potential bias of relating hate speech with female gender tweets; when the tweets are modified from pertaining to females, the tweets are predicted as not hate. Different topics are used to modify the tweets such as medicine where the contrast discusses a patient of unknown gender. The third row illustrates insight into the black box model that requires an interaction of words. The word ``immigration" by itself is not necessarily aligned with hate speech but ``illegal immigration" is more likely aligned with such speech as shown by the prediction. Adding attributes about money and science are used to explain how the tweet can be changed to not hate. The last two rows make the same point as the first two rows but in the reverse direction; modifying tweets that are not hateful by adding female connotations can easily change the prediction to hate. This is a potential bias of the black box model that should be investigated and is how one can benefit from using contrastive explanations. The insight from the attributes is that there are different topics through which the bias can be introduced. Moreover, the last example shows again that a single perturbation is not enough; in this case, an insertion and replacement are required to find a contrast showing that while the addition of ``women" biases the classifier to predict hate, the interaction of words is important as an additional insertion is required.

\noindent\textbf{NLI}. The Natural Language Inference \cite{nli} dataset contains samples of two short ordered texts, and the labels are either contradiction if the second text contradicts the first, neutral if the two texts do not contradict or imply one another, or entailment if the second text is a logical consequence of the first text.

Table \ref{tab:nli} illustrates CAT applied to five example texts from the NLI dataset. The first row shows an entailment that was modified to a contradiction by replacing the word ``break" with ``lawn". While this would be the explanation offered by a typical counterfactual method, CAT additionally shows that the topic of electronics (often associated with the word ``break") was removed. Such insight can offer more clarity as to why the contrast was predicted a contradiction rather than neutral, which seems more likely until we learn that the electronics topic that has nothing to do with the hypothesis was removed from the text. In row two, the change of ``chrome" to ``rust" is attributed to adding the space topic (as rust is an important issue in space exploration) and removed the graphics and electronics topics associated with chrome(books or web browsers). In row three, the difference of children being a part of a tournament versus simply watching the tournament is attributed to a reduction of the entertainment topic (and similarly in row four for playing a guitar versus stealing a guitar). In row five, the change of ``naps" to ``photos" is attributed to adding the graphics topic, which makes sense and helps build trust in the model.

\eat{
\textbf{DBPedia}. This dataset is derived from Wikipedia which focuses mainly on location and organizations of 14 classes. The dataset contains 560K training and 70K test examples. 

\textbf{Yelp}. The dataset is composed on informal text containing reviews of business of two classes, namely positive and negative. We use a filtered version of YELP Polarity dataset by choosing sentences of length upto 15 words. The filtered dataset contains 250K negative and 350K positive ones. 
}

==> Contrastive Attributed Text Explanation/intro.tex <==
% %!TEX root = main_v0.tex
% %%%
% %%% 							Introduction
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
%\vspace{-0.3cm}
\centering
\caption{Contrastive explanations are shown for a state-of-the-art method GYC, our method CAT and an ablation of our method called CAT-na that uses no attributes to explain predictions on two sentences from the AGNews dataset. The \textcolor{red}{red} highlighting indicates text that has changed in the contrastive explanation. Both inputs were classified as Sci-Tech while all contrastive sentences were classified as Business. In addition to these changes, CAT outputs the attributes (or subtopics) that it thinks were added/removed from the input to create the contrast. For instance, in the first example it is easy to to see that the added word ``ticket" could relate to ``Travel" and ``Sale", while the removed word ``server" from the input relates to ``Computers". Similarly, ``tax" in the second example could correspond to ``Entertainment" or ``Politics", while ``file" corresponds to software files that are often encrypted and hence to ``Cryptography".  As can be seen, CAT provides much closer and meaningful contrasts, where the attribute information provides further insight into what subtopics were added/removed to produce the contrast. This can unequivocally help appropriate trust in a model.}
\label{tab:introeg}
\begin{tabular}{|p{3.0cm}|p{3.0cm}|p{3.0cm}|p{2.2cm}|p{3.0cm}|}
  \hline
  \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Input}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{GYC}}} & \multicolumn{2}{c|}{\textbf{CAT}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{CAT-na}}} \\ \cline{3-4}
& &\multicolumn{1}{c|}{Contrast} & \multicolumn{1}{c|}{Attributes} & \\
 \hline
  Global server sales on the rise & Global server sales on \textcolor{red}{Friday, October} & Global \textcolor{red}{ticket} sales on the rise & $+$Travel, $+$Sale, $-$Computer &Global \textcolor{red}{drug} sales on the rise \\
 \hline
  Movie Studios to sue illegal film file traders & Movie Studios to sue \textcolor{red}{juveniles psychiatrically} & Movie Studios to sue illegal film \textcolor{red}{tax} traders &
  $+$Entertainment, $+$Politics, $-$Cryptography & Movie studios to sue illegal \textcolor{red}{insurance} file traders\\
 \hline
 \end{tabular}
 \vspace{-0.25cm}
 \end{table*}

Explainable AI (XAI) has seen an explosion of interest over the last five years or so, not just in AI research \cite{molnarbook,arya2019explanation}, but also in the real world where governments \cite{gdpr,xai} and industry \cite{umang} have made sizeable investments. The primary driver for this level of interest has been the inculcation of deep learning technologies \cite{gan}, which are inherently black box, into decision making systems that affect millions of people. Trust thus has become a central theme in relying on these black box systems, and one way to achieve it is seemingly through obtaining (posthoc) explanations.

Although many feature-based \cite{lime,unifiedPI,saliency} and exemplar-based methods \cite{proto,infl,l2c} have been proposed to explain local instance level decisions of black box models, contrastive/counterfactual explanations have seen a surge of interest recently \cite{gdpr-wachter,CEM,gyc,CEM-MAF,mice}. One reason for this is that
contrastive explanations are viewed as one of the main tools to achieve recourse \cite{algorec}. 

Given this surge of interest and its importance in recourse, in this paper, we propose a novel method Contrastive Attributed explanations for Text (CAT) which provides contrastive explanations for natural language data, a modality that has received comparatively less attention when it comes to these type of explanations. We show that our method produces fluent contrasts and possesses an additional novel twist not seen in prior works. As such, our method also outputs a minimal set of semantically meaningful attributes that it thinks led to the final contrast. These attributes could be subtopics in a dataset, different from the class labels, that characterize a piece of text or the attributes could even be obtained from a different dataset. Our approach is to leverage these attributes by building models (viz. classifiers)
for them and then using these classifiers to guide the search for contrasts in the original task. To better understand what CAT offers, consider the examples provided in Table \ref{tab:introeg}. Here we show two example sentences from the AG News dataset \cite{AgNews2015}, which were classified as Sci-Tech by our neural network black box (BB) model (details in Section \ref{sec:exp}). Each explanation method generates a contrast in the class Business where the other choices were World and Sports. As can be seen, our method CAT produces a closer contrast than a recent method termed Generate Your Counterfactuals (GYC) \cite{gyc}. 

A key novelty is that CAT provides additional information in terms characteristic attributes it thinks the contrast sentence belongs to (indicated by $+$ sign), while also indicating characteristics it thinks are no longer applicable (indicated by $-$ sign). These attributes were obtained from the 20 Newsgroup dataset \cite{AgNews2015} and the Huffpost News-Category dataset \cite{news_category}, where we trained classifiers for 42 such attributes (20 Newsgroup classes $+$ 22 Huffpost classes), and used them to regularize our search for the contrastive text. Our method picks a few relevant attributes that guide the generation of the contrast, and the attributes in themselves provide additional insight into the functioning of the black box model. This is confirmed through a user study conducted over 37 participants for which the results are reported in section \ref{sec:human}. Users found it easier to predict the class of the input sentence given our explanation over GYC and an ablation of our method, called CAT with no attributes (CAT-na), and moreover, users qualitatively preferred our method in terms of understandability, sufficiency, satisfiability and completeness on a five point Likert scale.

It is important to note that there are various ways to generate text using different language models (GPT-2, BERT, T5, etc.) and even different techniques on how infilling might be performed (forward or bi-directional). The key idea of guiding the generation of contrasts through attributes can be considered for other recent methods, whether the contrast is learned through differentiable optimization \cite{gyc} or through combinatorial search \cite{mice}. %We intend to release the source code for  future research.

As such, our contributions are as follows:
\begin{enumerate}
    \item CAT introduces the idea of using attributes to drive the generation of text contrastives. This contribution is both conceptual as it brings new insight to the user as well as methodological as it leads to user-preferred contrasts as seen in the user study.
    \item We qualitatively evaluate CAT through many examples on three different datasets from different domain tasks.
    \item We quantitatively evaluate CAT over other methods in terms of flip rate, content preservation, fluency, Levenstein distance and efficiency.
    \item We demonstrate the utility of CAT through a user study that asks users to determine a model's prediction on an instance given an explanation. The user study compares CAT with GYC and an ablation of our method CAT-na.
\end{enumerate}
% \noindent 1. CAT introduces the idea of using attributes to drive the generation of text contrastives. This contribution is both conceptual as it brings new insight to the user as well as methodological as it leads to user-preferred contrasts as seen in the user study.

% \noindent 2. We qualitatively evaluate CAT through many examples on three different datasets from different domain tasks.

% \noindent 3. We quantitatively evaluate CAT over other methods in terms of flip rate, content preservation, fluency, Levenstein distance and efficiency.

% \noindent 4. We demonstrate the utility of CAT through a user study that asks users to determine a model's prediction on an instance given an explanation. The user study compares CAT with GYC and an ablation of our method CAT-na.

\eat{
\begin{table*}[htbp]
%\vspace{-0.3cm}
\centering
\caption{Below we see contrastive explanations for a state-of-the-art method GYC, our method CAT and an ablation of our method without using attributes CAT-na for two sentences from the AGNews dataset. The \textcolor{red}{red} highlighting indicates the text that has changed in the contrastive explanation. The inputs were classified as Sci-Tech, while the contrasts for the different methods are all classified as Business. For CAT besides these changes we also see the attributes (or subtopics) that it thinks were added/removed from the input to create the contrast. For instance, in the first example it is easy to to see that the added word ``ticket" could relate to ``Travel" and ``Sale", while the removed word ``server" from the input relates to ``Computers". Similarly, ``tax" in the second example could correspond to ``Entertainment" or ``Politics", while ``file" corresponds to software files which many times are encryted and hence to ``Cryptography".  As can be seen CAT provides much closer and meaningful contrasts, where the attribute information provides further insight into what subtopics were added/removed to produce the contrast. This can unequivocally help appropriate trust in a model.}
\label{tab:introeg}
\begin{tabular}{|p{4cm}|p{4cm}|p{4cm}|p{4cm}|}
  \hline
   \textbf{Input} & \textbf{GYC} & \textbf{CAT} & \textbf{CAT-na} \\
 \hline
  Global server sales on the rise & Global server sales on \textcolor{red}{Friday, October} & Global \textcolor{red}{ticket} sales on the rise & Global \textcolor{red}{drug} sales on the rise \\
  &&&\\
 && Attributes: $+$Travel, $+$Sale, $-$Computer &\\
 \cline{1-4}
  Movie Studios to sue illegal film file traders & Movie Studios to sue \textcolor{red}{juveniles psychiatrically} & Movie Studios to sue illegal film \textcolor{red}{tax} traders &
  Movie studios to sue illegal \textcolor{red}{insurance} file traders\\
 &&&\\
 && Attributes: $+$Entertainment, $+$Politics, $-$Cryptography&\\
 \hline
 \end{tabular}
 \end{table*}
 }
 

%\begin{table*}[htbp]
%\begin{tabular}{|c|l|l|}
%\multicolumn{1}{c}{}& \multicolumn{1}{c}{\textbf{Example 1}} & \multicolumn{1}{c}{\textbf{Example 2}} \\
%\hline
%\textbf{Input} & Global server sales on the rise & Movie Studios to sue illegal film file traders \\ \hline
%\textbf{GYC} & Global server sales on \textcolor{red}{Friday, October} & Movie Studios to sue \textcolor{red}{juveniles psychiatrically} \\ \hline
%\textbf{CAT} & Global \textcolor{red}{ticket} sales on the rise & Movie Studios to sue illegal film \textcolor{red}{tax} traders \\ \hline
%\textbf{CAT Attributes} & +Travel, +Sale, -Computer & +Entertainment, +Politics, -Cryptography\\ \hline
%\textbf{CAT-na} & Global server sales on the rise & Movie Studios to sue illegal film file traders \\ \hline
%\textbf{Input Pred.} & \multicolumn{2}{c|}{Sci-Tech} \\ \hline
%\textbf{Contrast Pred.} & \multicolumn{2}{c|}{Business} \\ \hline

%\hline

%\end{tabular}

%\end{table*}





==> Contrastive Attributed Text Explanation/related_work.tex <==
%!TEX root = main.tex

%%% 							Concluding Remarks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
Regarding the explanations of machine learning predictions on text data, a recent survey \cite{xainlp_survey} considered 50 recent explainability works for natural language processing, and moreover only methods that ``justify predictions" rather than understanding ``a model's behavior in general". Our intention is also to explain individual predictions. Little work has been done for global explainability with respect to text classification; \cite{lime} suggests using various ``representative" local predictions to get a global understanding of model behavior. The vast majority of explainability techniques found by \cite{xainlp_survey} fall under local explainability.

Local methods can be divided among post-hoc methods that explain a fixed model's prediction and self-explainable methods where the model is itself understandable; our focus is on the former. One large group of explainability methods are feature based where the explanation outputs some form of feature importance (i.e., ranking, positive/negative relevance, contributions, etc.) of the words in text \cite{dknn_text,dknn,inputreduction,patternattribution_text,lime,melis_jaakkola_2017}. %\cite{dknn_text} apply k-nearest neighbors to a representation based on the output of each layer of a neural network (called deep k-nearest neighbors by \cite{dknn}) and assign feature importance by removing one word from the text at a time and observing which word most greatly affects the drop in ``conformity" (i.e., percentage of agreement) to its nearest neighbors. This work builds on the idea of input reduction \cite{inputreduction} which greedily removes words for which the removal of has least impact on the prediction and outputs the minimal set of words remain and maintain the same prediction as the original text. \cite{patternattribution_text} apply Pattern Attribution of \cite{patternet} (which improves on layer-wise relevance propogation of \cite{bach2015pixel} designed for image recognition) to the text domain to assign positive and negative contributions to words in Amazon reviews. 
%Another group of local post-hoc methods are surrogate models where one trains an interpretable model over perturbed instances of the original input and generates an explanation from the surrogate model. \cite{lime} uses linear surrogate models and obtains positive/negative relevance of features from the weights of the linear model. It is applicable to image, tabular and text (given a bag-of-words representation). \cite{melis_jaakkola_2017} use VAE \cite{vae_kingma} to account for semantics when generating perturbed sentences, use logistic regression to estimate class likelihoods given all tokens leading to a dense bipartite graph, and apply a graph partitioning method constrained by cut capacities to output a sparse bipartite graph (the surrogate model) that shows which tokens in the original sample are causal of which outputs. This technique was applied to machine translation and dialogue systems.
Other types of local post-hoc explanations include exemplar based \cite{proto,infl,l2c} that output similar instances to the input.% and saliency methods \cite{saliency} that output some form of the derivative of the output with respect to the input features. %There is a large literature on such methods but the majority focus is not on text as shown by the lack of citations in the survey \cite{xainlp_survey}. 

Amongst local methods our focus is on contrastive/counterfactual methods \cite{CEM, gyc, CEM-MAF} that modify the input such that the class changes and explains the prediction as ``If the sample were modified by $X$, the prediction would have been $Y$ instead," where $X$ is a change to the input and $Y$ is a new class. Such explanations are complementary to the other methods discussed above. They offer different types of intuition and thus should be used in conjunction with rather than instead of counterfactuals. \cite{CEM-MAF} learn contrasts using latent attributes, but specifically for color images. Their approach does not readily translate to text as humans do not perceive minor unrealistic parts of a generated image, whereas any nuance in text is easily noticed. Thus, generating (fluent) contrasts for text models is inherently much more challenging.

The most relevant comparisons to our work are GYC \cite{gyc} and MICE \cite{mice}. GYC builds on the text generation of \cite{pplm} by learning perturbations to the history matrix used for language modeling that are also trained to reconstruct input from the generated counterfactuals. A diversity regularization term ensures that this does not result in counterfactuals that are identical to the input. A more recent work MICE masks and replaces important words selected by \cite{saliency} in order to flip the prediction. MICE requires fine-tuning their language model to each dataset, which is a significant overhead especially given the fact that we are simply generating local explanations versus our CAT framework. Not to mention in many real applications (sufficient) data may not be available to fine tune explanations \cite{macem}. Both GYC and MICE works are targeted, i.e., the user must decide what class the counterfactual should be in as opposed to CAT which automatically decides the contrast class. 

Other recent methods are POLYJUICE \cite{polyjuice} and a contrastive latent space method \cite{jacovi}. The former is a human-in-the-loop method requiring supervision about the type of modification to be performed to the text such as negation, word replacement, insertion, deletion, and is not catered towards explaining a specific classifier by automatically finding the appropriate edits. The latter does not generate contrastive text but rather highlights (multiple) words in the input text that are most likely to alter the prediction if changed, where again the target class has to be provided. Further, \cite{jacovi} assume access to encodings from the second-to-last layer of the model being explained, and is thus not a black box method like CAT. %Similar to MICE, POLYJUICE uses masks to infill and selects generated counterfactuals that are most fluent as measured by the change in likelihood from that of the original text. 
Our focus being automated contrastive explanation generation, we compare with GYC and MICE, i.e., methods designed towards explaining a classifier, where a valid contrast is also generated. The value of CAT versus GYC and MICE comes from the output of (hidden) subtopics that are added/removed from the original text to create the contrast, giving important intuition that is missing from these other methods. This is confirmed through two user studies we conduct and qualitative examples we provide. The attribute classifiers built to predict these subtopics also aid in creating better contrasts. Moreover, as will be evident, such attribute classifiers can be used across datasets, thus precluding the need for each dataset to contain such attributes. Furthermore, topic models or autoencoders could be used to divulge such attributes.%We combine the infilling ideas above with the leveraging of latent features done in \cite{CEM-MAF} (which was only applied to image data). 



==> Contrastive Attributed Text Explanation/supp_arxiv_emnlp.tex <==
% \clearpage
%\section*{Supplement for CAT}
\appendix
\section*{Appendix}


\section{Hyperparemeter tuning for CAT}\label{sec:hyperparam}
Since no ground truth exists for our contrastive explanations, hyperparameters for CAT objective (given in Eq.\ref{eqn:main}) were tuned qualitatively by observation. It is important to consider that, in practice a user will only need to tune the hyperparameters once at the beginning and will then be able to generate explanations for an arbitrary number of instances from the dataset. Our tuning led to the following values which we used across datasets: We kept highest weights for $\lambda = 5.0$ to make sure that perturbed sentences have a label different from that of original sentence. We used mean of BERT logits of words inserted/replaced as a surrogate for $p_{LM}(x')$ with regularization parameter $\eta$ set to be $1.0$ and regularization parameter $\nu$ for Levenshtein distance set to $2.0$. $\beta$ was set to $3.0$. The threshold for predicting addition or removal of attributes $\tau$, we used two values. For binary attribute classifiers from the Huffpost News dataset, we set $\tau = 0.3$, and for multiclass attribute classifiers trained on the 20 Newsgroup dataset, we set $\tau=0.05$.

We took 50 randomly selected examples from the training set, generated explanations and evaluated them manually to choose hyperparameters which is similar to prior works \cite{CEM-MAF, gyc}. The boundary values for hyperparameter search were $\lambda \in [4,10]$, $\beta \in [1,5]$, $\eta \in [0.5, 2]$, $\nu \in [1,4]$, and $\tau \in [0.01, 0.5]$.
With more examples for tuning we would expect better explanations, although we found this number to be sufficient.

\section{Attribute classifiers}\label{sec:attr}
In our experiments we created 42 attributes from Huffpost News-Category dataset\cite{news_category} and 20 Newsgroups \cite{kaggle20NewsGrp}.

News-Category dataset \footnote{\url{https://www.kaggle.com/rmisra/news-category-dataset}} has 41 classes of which we merged similar classes and removed those which weren't standard topic. For instance, classes ``\textit{food \& drink}" and ``\textit{taste}" was merged and labelled as a new class ``\textit{food}". At the end we obtained the following 22 classes: \textit{education, money, world, home \& living, comedy, food, black voices, parenting, travel, sports, women, religion, Latino voices, weddings, entertainment, crime, queer voices, arts, politics, science, fifty}, and \textit{environment}. We created 22 1-vs-all binary classifiers, so that the same sentence can have multiple classes. To alleviate the class imbalance issue in training these binary classifiers we sampled fewer instances uniformly at random from the negative classes making sure that the number of negative instances are no more than $80\%$ of the training data.

The 20 Newsgroup dataset \footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.fetch_20newsgroups.html}} has the following 20 classes: \textit{atheism, graphics, ms-windows.misc, computer, mac.hardware, ms-windows.x, forsale, autos, motorcycles, baseball, hockey, cryptography, electronics, medicine, space, christian, guns, mideast, politics}, and \textit{religion}. A distilbert multi-class classifier was trained on this data.

All attribute classifiers were trained with DistliBERT base \footnote{\url{https://huggingface.co/distilbert-base-uncased}} for $10$ epochs using the Adam optimizer with a learning rate of $5\times 10^{-5}$, weight decay of $0.01$, and a batch size of $16$. Each of the models were trained using NVIDIA V100 GPUs in under 12 hours.

\section{Text classifiers}\label{sec:classifier_details}
We conducted experiments on two sets of text classifiers trained on four datasets: One set to compare CAT with GYC and another to compared CAT with MICE. All experiments were run on NVIDIA V100 GPUs.

For experiments comparing CAT with GYC\cite{gyc}, we trained model with the same architecture as the one used in their paper. This model is composed of an \textit{EmbeddingBag} layer followed by a linear layer, a \textit{ReLU} and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss. A GPT2 tokenizer \footnote{\url{https://huggingface.co/gpt2-medium}} was used to convert text into bag of words. The models were trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$.

For experiments comparing CAT with MICE\cite{mice}, we used author provided implementation\footnote{\url{https://github.com/allenai/mice}} to train models with \texttt{AllenNLP} \cite{allennlp}. This architecture is composed of a \textit{RoBERTa-base} model with a linear layer. For all four datasets the models were trained for $5$ epochs with batch size of $8$ using Adam optimizer with a learning rate of $4e-05$, weight decay of $0.1$, and slanted triangular learning rate scheduler with cut frac $0.06$.

\section{Datasets}\label{sec:datasets}
We performed experiments on 4 datasets: AgNews\cite{AgNews2015}, NLI\cite{nli}, DBpedia \cite{Lehmann2015DBpediaA}, and Yelp\cite{Shen2017}. AgNews dataset was taken from Kaggle website \footnote{\url{https://www.kaggle.com/datasets/amananandrai/ag-news-classification-dataset}} and rest three datasets from \textit{huggingface datasets}\cite{hf_datasets}.

\textbf {AgNews}. The dataset is from a real-world news domain which contains short news headlines and bodies from four new categories - world, business, sports, and sci-tech. It contains ~30K training and ~1.9K test examples per class, comprising of ~128K samples. Our experiments focus on explanations for predicting the class from the headlines.

\textbf{NLI}. The Natural Language Inference \cite{nli} dataset\footnote{\url{https://huggingface.co/datasets/snli}} contains samples of two short ordered texts, and the labels are either \textit{contradiction} if the second text contradicts the first, \textit{neutral} if the two texts do not contradict or imply one another, or \textit{entailment} if the second text is a logical consequence of the first text. The dataset contains ~550K training, 10K test and 10K validation examples.

\textbf{DBpedia}. This dataset is a subset of original DBpedia data which is a crowd-sourced community effort to extract structured information from Wikipedia. This dataset\footnote{\url{https://huggingface.co/datasets/dbpedia_14}} is constructed by picking 14 non-overlapping classes from DBpedia 2014 with 40K training and 5K test examples per class. Task here is to predict the class a DBpedia entry belong to. In our experiments we only use \textit{content} and drop the \textit{title} field provided with with the dataset.

\textbf{Yelp}. This is a binary sentiment classification dataset\footnote{\url{https://huggingface.co/datasets/yelp_polarity}} containing 560K highly polar reviews for training and 38K for testing. The dataset consists of reviews from Yelp which is extracted from the Yelp Dataset Challenge 2015.


% \singlecolumn[\centering\Large\bfseries Let the CAT out of the bag: \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext\\
% (Appendix) \par \medskip]
% \twocolumn[\centering\Large\bfseries Let the CAT out of the bag: \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext\\
% (Appendix) \par \medskip]

% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on four metrics: 1) \textbf{Flip} rate, ii) \textbf{Dist}(distance), iii) \textbf{Fluency}, iv) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev) for all the metrics for CAT.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|cccc|cccc}
% \multicolumn{9}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{4}{c|}{AgNews} &
%       \multicolumn{4}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Flip & Dist & Cont & Fluency &
%       Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.164 $  &$0.110 $  & $0.286$ &$0$  &$0.140$  &$0.105$  &$0.467$  \\
%       std. dev.(CAT) &$0$  &$0.098 $  &$0.084 $  & $0.105$ &$0$  &$0.100$  &$0.076$  &$0.134$  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{4}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       &Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.132 $  &$0.115 $  & $0.344$ \\
%       std. dev.(CAT) & $0$  &$0.059 $  &$0.069 $  & $0.064$ \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}

\begin{table*}[!]
 \centering
% \caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
% }
\caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC with CAT and MICE with CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC as well than MICE. We also report standard deviation (std. dev.) for all metrics for CAT, GYC and MICE, which together with the means reported in the main paper, are used to run the t-tests.
}
 \label{tab:quant_stat}
\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
	\multicolumn{7}{c}{\textbf{Embedding Bag based Classifier}}\\ 
\hline
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.164   &0.110   &0.286  &0.140  &0.105  &0.467  \\
      std. dev. (CAT)   &\textbf{0.098}  &\textbf{0.084} &\textbf{0.105 } &\textbf{0.100} &\textbf{0.076} &\textbf{0.134}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|ccc|ccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC)  &0.132   &0.115   &0.344 \\
%       std. dev.(CAT)   &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule

\multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{Dbpedia} &
      \multicolumn{3}{c}{NLI} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
      & Dist & Cont & Fluency &
      Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.132   &0.115   &0.344   &\multicolumn{3}{|c}{NR}  \\
      std. dev. (CAT)    &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} &\textbf{0.323} &\textbf{0.010} &\textbf{0.033}  \\
      \bottomrule
  \end{tabular}
  
  
% \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Method} &
%       \multicolumn{4}{c}{Hate Speech} \\
%       & Flip & Dist & Cont & Fluency\\
%         \midrule
%       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
%       \bottomrule
%   \end{tabular}

\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
	\multicolumn{7}{c}{\textbf{Roberta based Classifier}}\\ 
\hline
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (MICE)   &\textbf{0.182}   & \textbf{0.121}   &0.196  &0.174  &0.109  &0.208  \\
      std. dev. (MICE-nft)   &0.307   &0.209   &0.224  &0.240  &0.154  &0.212  \\
      std. dev. (CAT)   &0.307  &0.209 & \textbf{0.144}  & \textbf{0.084} & \textbf{0.044} &\textbf{0.098}  \\
      
    %   std. dev. (CAT-na)   &\textbf{0.101}  &\textbf{0.072}  &\textbf{0.145} &\textbf{0.0} &\textbf{0.0} &\textbf{0.0}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|ccc|ccc}
 \multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{Dbpedia} &
      \multicolumn{3}{c}{NLI} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
      & Dist & Cont & Fluency &
      Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev.(MICE)  &0.151   &0.077   &0.168  &0.132   &0.109   &0.131  \\
      std. dev.(MICE-nft)  &0.200  &0.160  &0.160 &\textbf{0.164} &0.088 &0.143 \\
      std. dev.(CAT)   &\textbf{0.058}  & \textbf{0.039}  & \textbf{0.071} &\textbf{0.037} &\textbf{0.013} &\textbf{0.054}  \\
      \bottomrule
      
      
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(MICE)  &0.151   &0.077   &0.168 \\
%       std. dev.(MICE-nft)  &0.200  &0.160  &0.160 \\
%       std. dev.(CAT)   &0.0  &0.0  &0.0 \\
      
%     %   std. dev.(CAT-na)   &\textbf{0.0}  &\textbf{0.0}  &\textbf{0.0} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
  \end{tabular}
  \label{tab:quant_stat}
\end{table*}


\section{Quantitative Evaluation Statistics}\label{sec:quant_stat}
Table \ref{tab:quant} (in the main paper) shows the performance evaluation of our proposed approach, CAT, on five different datasets and $2$ classifier models, namely Embedding Bag based classifier and Roberta based classifier models. It was noted that CAT outperformed GYC  and MICE over AgNews, Yelp and Dbpedia by statistically significant margins on respective model. Recall that GYC usage Embedding Bag based classifier model and MICE usage Roberta based classifier. Therefore, we implemented both the classifier models with CAT to compare both GYC and MICE.  We verify this statement in Table \ref{tab:quant_stat} where we report pairwise t-tests comparing the means for CAT with GYC and CAT with MICE and standard deviation of CAT, GYC, MICE for each metric and dataset.  The improvement of CAT over GYC and MICE is observed to be statistically significant across all metrics. We do not report additional statistics for the flip rate metric as CAT always produces a contrastive sentence with a flipped class label unlike GYC or MICE which sometimes fails to flip.

% \section{Additional Setup Details}
% All experiments were run on NVIDIA V100 GPUs. Of the four data sets experimented in the paper, models trained on NLI \eat{and the Hate Speech dataset} were directly taken from the huggingface website\footnote{\url{https://huggingface.co/roberta-large-mnli} \eat{\\\url{https://huggingface.co/cardiffnlp/twitter-roberta-base-hate}}}. %Yelp, AgNews, and DBpedia were trained 
% %\textcolor{blue}{Amar to add details of BoW models such as architecture, optimizer, learning rate etc.}
% The black box models for AgNews, DBPedia and Yelp is composed of an \textit{EmbeddingBag} layer followed by a linear layer, a \textit{ReLU} and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss for 4, 14 and 2 classes for AgNews, DBPedia and Yelp, respectively. A GPT2 tokenizer \footnote{\url{https://huggingface.co/gpt2-medium}} was used to convert text into bag of words. We choose this model architecture to match the models used in GYC \cite{gyc}. The model is trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$. Our code is licensed under Apache-2.0.

\section{Additional Information for User Study}
Figure \ref{fig:userinstr} shows screenshots of user study 1, including the instructions and example questions for the three different methods discussed in the study. The same instructions and format was used for user study 2, except that we asked five task oriented questions (rather than seven) per explainer as there were four explainers (as opposed to 3) keeping the total number of questions to be 24, and thus keeping the overall effort of both user studies roughly the same for participants. For the users the methods were named as Explainer A, B and C, where they correspond to GYC, CAT, and CAT-na respectively for user study 1. For user study 2, Explainer A, B, C and D corresponded to MICE, MICE-nft, CAT and CAT-na. Some users also left optional comments at the end of the user study which we list here:

\begin{itemize}
    \item ``I found the questions confusing... What is complete, sufficient and understandable explanation in a word change? Also, in each example, what was I supposed to guess, the category of the article or the possible prediction of the method? Are those things different?'' (Study 1)
    \item ``Explainer A was pretty bad, explainer B was very good, and explainer C was reasonably good.'' (Study 1)
    \item ``Explainer b was the best. The q\&a at the end of each page allows multiple choices per row, which is bad. Each question should remove the modified classification as an option (if the modified sentence is World, I shouldn't be allowed to choose World). Early on the survey should state clearly that there are only 4 categories (business/sci-tech/sports/world) which I didn't know right away, I expected each question have 4 different options, and knowing this might have helped me understand what we're doing here better. The opening text was very confusing.'' (Study 1)
    \item ``I found B to be the best one.'' (Study 1)
    \item ``nice survey'' (Study 1)
    \item ``the additional info in explanation C was useful'' (Study 2)
\end{itemize}



\begin{figure*}[htbp]
\centering
 \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/CAT_instr.png}
        \caption{}
    \end{subfigure}
     \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/likert_ss.png}
        \caption{}
    \end{subfigure}\\
   %\vspace{0.2cm}
   \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/gyc_ss.png}
        \caption{}
    \end{subfigure}
   \hspace{0.1\textwidth}
   \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/cat_ss.png}
        \caption{}
    \end{subfigure}
  \caption{In (a) we show the instructions for the survey. In (b) we see the qualitative questions. In (c) and (d) we see the task oriented questions for GYC and CAT respectively.} 
\label{fig:userinstr}
%\vspace{-0.3cm}
\end{figure*}

\section{Additional Qualitative Examples}\label{sec:qualitative_examples}
Table \ref{tab:extra_examples} offers at least five more examples of contrastive explanations from each dataset. Additional insight can be gained from the attributes; in the first row, adding travel-related text can flip the class from business to world, i.e., the article was predicted business because if it was more about travel it would have been predicted as world. This type of explanation adds extra intuition as opposed to only being given the replacement of words, ``oil" to ``winds" in this case. As can also been seen, insight is also a function of using attributes that have a relationship to the dataset and task. For example, attributes derived from news sources are often not helpful for explaining sentiment classifiers (e.g., Yelp) for which sentiment is often flipped by the negation of the text. This is to be expected; good explanations require good attributes.

\begin{table*}[htbp]
\centering
\small
\caption{Extra contrastive explanation examples from four datasets: AgNews, NLI, DBPedia, and Yelp.}
\label{tab:extra_examples}
% \begin{tabular}{|p{7cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\begin{tabular}{|p{5.75cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Input/CAT}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Attribute Changes}}}  & \multicolumn{1}{c|}{\textbf{Input}} & \multicolumn{1}{c|}{\textbf{Contrast}}
& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}}\\
   &  & \multicolumn{1}{c|}{\textbf{Pred}}  &\multicolumn{1}{c|}{\textbf{Pred}}&  \\ \hline

\st{Oil} \textcolor{red}{Winds} Up from 7-Week Lows on U.S. Weather & \multicolumn{1}{c|}{+travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{world} & AgNews \\ \hline

New Hummer Is Smaller, Cheaper and Less \st{Gas} \textcolor{red}{cpu} Hungry & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -travel, \\-space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ 
\hline

Perfect start for France in \st{Federation} \textcolor{red}{Microsoft} Cup & \multirow{2}{*}{\shortstack{+cryptography, -motorcycles, \\-hockey, -space, -politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\ \hline
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey}& \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\st{Kuwait} \textcolor{red}{Source}: Fundamentalists Recruiting Teens (AP) &  \multicolumn{1}{c|}{+guns, religion, -mideast}& \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\multirow{2}{*}{Harry \st{in nightclub} \textcolor{red}{inflight} scuffle}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+sports, +space, -religion, \\-cryptography, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline
\eat{
I thought you \textcolor{red}{ladies} were leaving the country you washed up \$\$\$\$ \$\$\$\$? & \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -cryptography}}& \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

Such crimes must attract severest punishment,say Min Jail term of 25Y. If they r \st{illegal} \st{migrants} \textcolor{red}{convicted}, force them to leave the Country immediately& \multicolumn{1}{c|}{\multirow{3}{*}{+atheism, -politics}} & \multicolumn{1}{c|}{\multirow{3}{*}{hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{Hate}} \\ \hline

\multirow{2}{*}{\st{@brianstelter} \textcolor{red}{she} is a complete \st{joke} \textcolor{red}{\$\$\$\$} ! if you see...}& 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +cryptography, \\-sports, -politics}} }& \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Do \st{you} \textcolor{red}{chicks} ever \st{rap} \textcolor{red}{talk} in your whitest voice possible or is that just me?& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+parenting, +atheism, +politics \\-world, -sports, -arts}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

\st{There's} \textcolor{red}{Women} \textcolor{red}{get} no greater satisfaction than knowing you did it yourself' -me when someone asks me ... & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +entertainment, \\ +religion, -sports}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline
}
Five soldiers hold and aim their \st{weapons} \textcolor{red}{blades}. $<$/s$>$ The soldiers are \st{eating} \textcolor{red}{armed}.
& \multicolumn{1}{c|}{\multirow{2}{*}{-guns}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Skateboarder jumps of off dumpster. $<$/s$>$ a \st{bike} \textcolor{red}{young} rider in a race&
 \multicolumn{1}{c|}{\multirow{2}{*}{+world}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Two people walking down a dirt trail with backpacks on looking at \st{items} \textcolor{red}{map} they are carrying. $<$/s$>$ One is holding a map.
& \multicolumn{1}{c|}{\multirow{3}{*}{+space, -motorcyles, -electronics}}& \multicolumn{1}{c|}{\multirow{3}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

A brown and black dog is jumping to catch a red ball. $<$/s$>$ Two dogs are
\textcolor{red}{not} playing catch with their owner.
& \multicolumn{1}{c|}{\multirow{2}{*}{-arts}}& \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

A girl is standing in a field pushing up her hat with one finger and her hand is
covering most of her face. $<$/s$>$ A \st{girl} \textcolor{red}{boy} covers her face. 
& \multicolumn{1}{c|}{\multirow{3}{*}{+parenting, -medicine}}& \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

Channel Chaos is a 1985 Australian \st{film} \textcolor{red}{production} set at a TV station & \multicolumn{1}{c|}{\multirow{2}{*}{+electronics, -travel, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{film}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

\multirow{2}{*}{Dinik is a \st{village} \textcolor{red}{lake} in Croatia}
& \multicolumn{1}{c|}{\multirow{2}{*}{+medicine, +space, -mideast}}& \multicolumn{1}{c|}{\multirow{2}{*}{village}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{natural\\place}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

%\multirow{2}{*}{Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}}
Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}
& \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{plant}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{written\\work}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

ACTION is a bus service \st{operator} \textcolor{red}{based} in Canberra Australia
& \multicolumn{1}{c|}{\multirow{2}{*}{+autos, -electronics}}& \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{transport\\-ation}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

Jagjaguwar is an indie rock record \st{label} \textcolor{red}{musician} based in Bloomington Indiana 
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+space, +politics, -world \\-forsale, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{artist}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

he \st{really} \textcolor{red}{hardly} made our anniversary dinner entertaining memorable
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +sports, +cryptography \\-home\&living, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

they also have deep fried desserts if you're \st{brave} \textcolor{red}{poor} enough
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+medicine, -travel \\-religion, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

i \st{definitely} \textcolor{red}{never} will go back & \multicolumn{1}{|c|}{-entertainment} &\multicolumn{1}{c|}{positive}&\multicolumn{1}{c|}{negative}&\multicolumn{1}{c|}{Yelp} \\ \hline

\multirow{2}{*}{jesse is completely \st{rude} \textcolor{red}{perfect}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -entertainment, \\-medicine, -space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

\multirow{2}{*}{the pizza \st{sauce} \textcolor{red}{heaven} is also way too sweet} & 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +travel, +arts, +atheism \\+religion, -medicine, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline


\eat{
\multirow{2}{*}{Kazaa Owner Cheers \st{File} \textcolor{red}{Salary}-Swapping Decision (AP)} \quad\quad\quad\quad\quad\quad\quad\quad & \multirow{2}{*}{\shortstack{+forsale, +baseball, +hockey,\\ -arts, -windows, -cryptography}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \\
\hline

New Human Species \st{Discovered} \textcolor{red}{influenza} & +medicine, -cryptography & \multicolumn{1}{c|}{sci-tech} & \multicolumn{1}{c|}{world} \\ \hline

US shows flexibility on \st{Israeli} \textcolor{red}{virtual} settlements & +arts, +cryptography, -mideast & \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} \\ \hline


\eat{Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey} & \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{business} \\ \hline}

Pace of U.S. \st{Factory} \textcolor{red}{population} Growth Climbs in Dec & \multicolumn{1}{c|}{+politics, -money, -travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{sci-tech} \\ \hline

It may take 146 years for Nigeria to wipe out \st{corruption} \textcolor{red}{funds} from \st{its} \textcolor{red}{bank} system going by the latest report ...\eat{by Transparency International (TI) which gave the country the third position among the most corrupt countries of the world} & \multicolumn{1}{c|}{\multirow{2}{*}{+ money, - politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} \\ \hline
}
\end{tabular}
 \end{table*}
 
%\section{Limitations}
%Since our explanation is based on BERT which is pretrained for natural languages, it might have difficulties with informal or non grammatical sentences such as those coming from tweets. However, the limilation  can be potentially alleviated by language model fine tuning on the relevant dataset, e.g. on a tweet dataset, or by using other language models that are tailored to specific use cases.


% Since our explanation is based on natural language model (BERT), it might have difficulties with informal or non grammatical sentences such as those coming from tweets. The reason is due to a dependency on BERT, but if issues arise, this could potentially be fixed with other language models that are tailored to specific usecases.

\eat{The main limitation to our CAT method is the need for attribute classifiers. However, as noted in the paper, the attributes can be derived from other sources of data and not necessarily be dependent on the data and model being explained. Furthermore, there are other methods to obtain attributes. Unsupervised methods such as LDA, VAEs, GANs could be leveraged to ascertain semantically meaningful attributes. The attribute classifier that appears in our loss function could be replaced by disentangled representations learned by VAEs \cite{DIP-VAE} or by topic models. This shows that CAT is not limited to only annotated datasets.} 







% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|ccc|ccc}
% \multicolumn{7}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{3}{c|}{AgNews} &
%       \multicolumn{3}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Dist & Cont & Fluency &
%       Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev. (MICE)   &0.182   &0.121   &0.196  &0.174  &0.109  &0.208  \\
%       std. dev. (MICE-nft)   &0.307   &0.209   &0.224  &0.240  &0.154  &0.212  \\
%       std. dev. (CAT)   &0.307  &0.209 &0.144  &0.0 &0.0 &0  \\
      
%     %   std. dev. (CAT-na)   &\textbf{0.101}  &\textbf{0.072}  &\textbf{0.145} &\textbf{0.0} &\textbf{0.0} &\textbf{0.0}  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(MICE)  &0.151   &0.077   &0.168 \\
%       std. dev.(MICE-nft)  &0.200  &0.160  &0.160 \\
%       std. dev.(CAT)   &0.0  &0.0  &0.0 \\
      
%     %   std. dev.(CAT-na)   &\textbf{0.0}  &\textbf{0.0}  &\textbf{0.0} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}


==> Contrastive Attributed Text Explanation/supp_emnlp.tex <==
% \clearpage
%\section*{Supplement for CAT}

\appendix
\twocolumn[\centering\Large\bfseries Let the CAT out of the bag: \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext\\
(Appendix) \par \medskip]

% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on four metrics: 1) \textbf{Flip} rate, ii) \textbf{Dist}(distance), iii) \textbf{Fluency}, iv) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev) for all the metrics for CAT.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|cccc|cccc}
% \multicolumn{9}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{4}{c|}{AgNews} &
%       \multicolumn{4}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Flip & Dist & Cont & Fluency &
%       Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.164 $  &$0.110 $  & $0.286$ &$0$  &$0.140$  &$0.105$  &$0.467$  \\
%       std. dev.(CAT) &$0$  &$0.098 $  &$0.084 $  & $0.105$ &$0$  &$0.100$  &$0.076$  &$0.134$  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{4}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       &Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.132 $  &$0.115 $  & $0.344$ \\
%       std. dev.(CAT) & $0$  &$0.059 $  &$0.069 $  & $0.064$ \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}

\begin{table*}[!]
 \centering
% \caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
% }
\caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC with CAT and MICE with CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC as well than MICE. We also report standard deviation (std. dev.) for all metrics for CAT, GYC and MICE, which together with the means reported in the main paper, are used to run the t-tests.
}
 \label{tab:quant_stat}
\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
	\multicolumn{7}{c}{\textbf{Embedding Bag based Classifier}}\\ 
\hline
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.164   &0.110   &0.286  &0.140  &0.105  &0.467  \\
      std. dev. (CAT)   &\textbf{0.098}  &\textbf{0.084} &\textbf{0.105 } &\textbf{0.100} &\textbf{0.076} &\textbf{0.134}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|ccc|ccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC)  &0.132   &0.115   &0.344 \\
%       std. dev.(CAT)   &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule

\multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{Dbpedia} &
      \multicolumn{3}{c}{NLI} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
      & Dist & Cont & Fluency &
      Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.132   &0.115   &0.344   &\multicolumn{3}{|c}{NR}  \\
      std. dev. (CAT)    &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} &\textbf{0.323} &\textbf{0.010} &\textbf{0.033}  \\
      \bottomrule
  \end{tabular}
  
  
% \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Method} &
%       \multicolumn{4}{c}{Hate Speech} \\
%       & Flip & Dist & Cont & Fluency\\
%         \midrule
%       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
%       \bottomrule
%   \end{tabular}

\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
	\multicolumn{7}{c}{\textbf{Roberta based Classifier}}\\ 
\hline
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (MICE)   &\textbf{0.182}   & \textbf{0.121}   &0.196  &0.174  &0.109  &0.208  \\
      std. dev. (MICE-nft)   &0.307   &0.209   &0.224  &0.240  &0.154  &0.212  \\
      std. dev. (CAT)   &0.307  &0.209 & \textbf{0.144}  & \textbf{0.084} & \textbf{0.044} &\textbf{0.098}  \\
      
    %   std. dev. (CAT-na)   &\textbf{0.101}  &\textbf{0.072}  &\textbf{0.145} &\textbf{0.0} &\textbf{0.0} &\textbf{0.0}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|ccc|ccc}
 \multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{Dbpedia} &
      \multicolumn{3}{c}{NLI} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
      & Dist & Cont & Fluency &
      Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev.(MICE)  &0.151   &0.077   &0.168  &0.132   &0.109   &0.131  \\
      std. dev.(MICE-nft)  &0.200  &0.160  &0.160 &\textbf{0.164} &0.088 &0.143 \\
      std. dev.(CAT)   &\textbf{0.058}  & \textbf{0.039}  & \textbf{0.071} &\textbf{0.037} &\textbf{0.013} &\textbf{0.054}  \\
      \bottomrule
      
      
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(MICE)  &0.151   &0.077   &0.168 \\
%       std. dev.(MICE-nft)  &0.200  &0.160  &0.160 \\
%       std. dev.(CAT)   &0.0  &0.0  &0.0 \\
      
%     %   std. dev.(CAT-na)   &\textbf{0.0}  &\textbf{0.0}  &\textbf{0.0} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
  \end{tabular}
  \label{tab:quant_stat}
\end{table*}


\section{Hyperparemeter tuning for CAT}\label{sec:hyperparam}
Since no ground truth exists for our contrastive explanations, hyperparameters for CAT objective (given in Eq.\ref{eqn:main}) were tuned qualitatively by observation. It is important to consider that, in practice a user will only need to tune the hyperparameters once at the beginning and will then be able to generate explanations for an arbitrary number of instances from the dataset. Our tuning led to the following values which we used across datasets: We kept highest weights for $\lambda = 5.0$ to make sure that perturbed sentences have a label different from that of original sentence. We used mean of BERT logits of words inserted/replaced as a surrogate for $p_{LM}(x')$ with regularization parameter $\eta$ set to be $1.0$ and regularization parameter $\nu$ for Levenshtein distance set to $2.0$. $\beta$ was set to $3.0$. The threshold for predicting addition or removal of attributes $\tau$, we used two values. For binary attribute classifiers from the Huffpost News dataset, we set $\tau = 0.3$, and for multiclass attribute classifiers trained on the 20 Newsgroup dataset, we set $\tau=0.05$.

We took 50 randomly selected examples from the training set, generated explanations and evaluated them manually to choose hyperparameters which is similar to prior works \cite{CEM-MAF, gyc}. The boundary values for hyperparameter search were $\lambda \in [4,10]$, $\beta \in [1,5]$, $\eta \in [0.5, 2]$, $\nu \in [1,4]$, and $\tau \in [0.01, 0.5]$.
With more examples for tuning we would expect better explanations, although we found this number to be sufficient.

\section{Attribute classifiers}\label{sec:attr}
In our experiments we created 42 attributes from Huffpost News-Category dataset\cite{news_category} and 20 Newsgroups \cite{kaggle20NewsGrp}.

News-Category dataset \footnote{\url{https://www.kaggle.com/rmisra/news-category-dataset}} has 41 classes of which we merged similar classes and removed those which weren't standard topic. For instance, classes ``\textit{food \& drink}" and ``\textit{taste}" was merged and labelled as a new class ``\textit{food}". At the end we obtained the following 22 classes: \textit{education, money, world, home \& living, comedy, food, black voices, parenting, travel, sports, women, religion, Latino voices, weddings, entertainment, crime, queer voices, arts, politics, science, fifty}, and \textit{environment}. We created 22 1-vs-all binary classifiers, so that the same sentence can have multiple classes. To alleviate the class imbalance issue in training these binary classifiers we sampled fewer instances uniformly at random from the negative classes making sure that the number of negative instances are no more than $80\%$ of the training data.

The 20 Newsgroup dataset \footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.fetch_20newsgroups.html}} has the following 20 classes: \textit{atheism, graphics, ms-windows.misc, computer, mac.hardware, ms-windows.x, forsale, autos, motorcycles, baseball, hockey, cryptography, electronics, medicine, space, christian, guns, mideast, politics}, and \textit{religion}. A distilbert multi-class classifier was trained on this data.

All attribute classifiers were trained with DistliBERT base \footnote{\url{https://huggingface.co/distilbert-base-uncased}} for $10$ epochs using the Adam optimizer with a learning rate of $5\times 10^{-5}$, weight decay of $0.01$, and a batch size of $16$. Each of the models were trained using NVIDIA V100 GPUs in under 12 hours.

\section{Text classifiers}\label{sec:classifier_details}
We conducted experiments on two sets of text classifiers trained on four datasets: One set to compare CAT with GYC and another to compared CAT with MICE. All experiments were run on NVIDIA V100 GPUs.

For experiments comparing CAT with GYC\cite{gyc}, we trained model with the same architecture as the one used in their paper. This model is composed of an \textit{EmbeddingBag} layer followed by a linear layer, a \textit{ReLU} and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss. A GPT2 tokenizer \footnote{\url{https://huggingface.co/gpt2-medium}} was used to convert text into bag of words. The models were trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$.

For experiments comparing CAT with MICE\cite{mice}, we used author provided implementation\footnote{\url{https://github.com/allenai/mice}} to train models with \texttt{AllenNLP} \cite{allennlp}. This architecture is composed of a \textit{RoBERTa-base} model with a linear layer. For all four datasets the models were trained for $5$ epochs with batch size of $8$ using Adam optimizer with a learning rate of $4e-05$, weight decay of $0.1$, and slanted triangular learning rate scheduler with cut frac $0.06$.

\section{Datasets}\label{sec:datasets}
We performed experiments on 4 datasets: AgNews\cite{AgNews2015}, NLI\cite{nli}, DBpedia \cite{Lehmann2015DBpediaA}, and Yelp\cite{Shen2017}. AgNews dataset was taken from Kaggle website \footnote{\url{https://www.kaggle.com/datasets/amananandrai/ag-news-classification-dataset}} and rest three datasets from \textit{huggingface datasets}\cite{hf_datasets}.

\textbf {AgNews}. The dataset is from a real-world news domain which contains short news headlines and bodies from four new categories - world, business, sports, and sci-tech. It contains ~30K training and ~1.9K test examples per class, comprising of ~128K samples. Our experiments focus on explanations for predicting the class from the headlines.

\textbf{NLI}. The Natural Language Inference \cite{nli} dataset\footnote{\url{https://huggingface.co/datasets/snli}} contains samples of two short ordered texts, and the labels are either \textit{contradiction} if the second text contradicts the first, \textit{neutral} if the two texts do not contradict or imply one another, or \textit{entailment} if the second text is a logical consequence of the first text. The dataset contains ~550K training, 10K test and 10K validation examples.

\textbf{DBpedia}. This dataset is a subset of original DBpedia data which is a crowd-sourced community effort to extract structured information from Wikipedia. This dataset\footnote{\url{https://huggingface.co/datasets/dbpedia_14}} is constructed by picking 14 non-overlapping classes from DBpedia 2014 with 40K training and 5K test examples per class. Task here is to predict the class a DBpedia entry belong to. In our experiments we only use \textit{content} and drop the \textit{title} field provided with with the dataset.

\textbf{Yelp}. This is a binary sentiment classification dataset\footnote{\url{https://huggingface.co/datasets/yelp_polarity}} containing 560K highly polar reviews for training and 38K for testing. The dataset consists of reviews from Yelp which is extracted from the Yelp Dataset Challenge 2015.


\section{Quantitative Evaluation Statistics}\label{sec:quant_stat}
Table \ref{tab:quant} (in the main paper) shows the performance evaluation of our proposed approach, CAT, on five different datasets and $2$ classifier models, namely Embedding Bag based classifier and Roberta based classifier models. It was noted that CAT outperformed GYC  and MICE over AgNews, Yelp and Dbpedia by statistically significant margins on respective model. Recall that GYC usage Embedding Bag based classifier model and MICE usage Roberta based classifier. Therefore, we implemented both the classifier models with CAT to compare both GYC and MICE.  We verify this statement in Table \ref{tab:quant_stat} where we report pairwise t-tests comparing the means for CAT with GYC and CAT with MICE and standard deviation of CAT, GYC, MICE for each metric and dataset.  The improvement of CAT over GYC and MICE is observed to be statistically significant across all metrics. We do not report additional statistics for the flip rate metric as CAT always produces a contrastive sentence with a flipped class label unlike GYC or MICE which sometimes fails to flip.

% \section{Additional Setup Details}
% All experiments were run on NVIDIA V100 GPUs. Of the four data sets experimented in the paper, models trained on NLI \eat{and the Hate Speech dataset} were directly taken from the huggingface website\footnote{\url{https://huggingface.co/roberta-large-mnli} \eat{\\\url{https://huggingface.co/cardiffnlp/twitter-roberta-base-hate}}}. %Yelp, AgNews, and DBpedia were trained 
% %\textcolor{blue}{Amar to add details of BoW models such as architecture, optimizer, learning rate etc.}
% The black box models for AgNews, DBPedia and Yelp is composed of an \textit{EmbeddingBag} layer followed by a linear layer, a \textit{ReLU} and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss for 4, 14 and 2 classes for AgNews, DBPedia and Yelp, respectively. A GPT2 tokenizer \footnote{\url{https://huggingface.co/gpt2-medium}} was used to convert text into bag of words. We choose this model architecture to match the models used in GYC \cite{gyc}. The model is trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$. Our code is licensed under Apache-2.0.

\section{Additional Information for User Study}
Figure \ref{fig:userinstr} shows screenshots of user study 1, including the instructions and example questions for the three different methods discussed in the study. The same instructions and format was used for user study 2, except that we asked five task oriented questions (rather than seven) per explainer as there were four explainers (as opposed to 3) keeping the total number of questions to be 24, and thus keeping the overall effort of both user studies roughly the same for participants. For the users the methods were named as Explainer A, B and C, where they correspond to GYC, CAT, and CAT-na respectively for user study 1. For user study 2, Explainer A, B, C and D corresponded to MICE, MICE-nft, CAT and CAT-na. Some users also left optional comments at the end of the user study which we list here:

\begin{itemize}
    \item ``I found the questions confusing... What is complete, sufficient and understandable explanation in a word change? Also, in each example, what was I supposed to guess, the category of the article or the possible prediction of the method? Are those things different?'' (Study 1)
    \item ``Explainer A was pretty bad, explainer B was very good, and explainer C was reasonably good.'' (Study 1)
    \item ``Explainer b was the best. The q\&a at the end of each page allows multiple choices per row, which is bad. Each question should remove the modified classification as an option (if the modified sentence is World, I shouldn't be allowed to choose World). Early on the survey should state clearly that there are only 4 categories (business/sci-tech/sports/world) which I didn't know right away, I expected each question have 4 different options, and knowing this might have helped me understand what we're doing here better. The opening text was very confusing.'' (Study 1)
    \item ``I found B to be the best one.'' (Study 1)
    \item ``nice survey'' (Study 1)
    \item ``the additional info in explanation C was useful'' (Study 2)
\end{itemize}



\begin{figure*}[htbp]
\centering
 \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/CAT_instr.png}
        \caption{}
    \end{subfigure}
     \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/likert_ss.png}
        \caption{}
    \end{subfigure}\\
   %\vspace{0.2cm}
   \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/gyc_ss.png}
        \caption{}
    \end{subfigure}
   \hspace{0.1\textwidth}
   \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/cat_ss.png}
        \caption{}
    \end{subfigure}
  \caption{In (a) we show the instructions for the survey. In (b) we see the qualitative questions. In (c) and (d) we see the task oriented questions for GYC and CAT respectively.} 
\label{fig:userinstr}
%\vspace{-0.3cm}
\end{figure*}

\section{Additional Qualitative Examples}\label{sec:qualitative_examples}
Table \ref{tab:extra_examples} offers at least five more examples of contrastive explanations from each dataset. Additional insight can be gained from the attributes; in the first row, adding travel-related text can flip the class from business to world, i.e., the article was predicted business because if it was more about travel it would have been predicted as world. This type of explanation adds extra intuition as opposed to only being given the replacement of words, ``oil" to ``winds" in this case. As can also been seen, insight is also a function of using attributes that have a relationship to the dataset and task. For example, attributes derived from news sources are often not helpful for explaining sentiment classifiers (e.g., Yelp) for which sentiment is often flipped by the negation of the text. This is to be expected; good explanations require good attributes.

\begin{table*}[htbp]
\centering
\small
\caption{Extra contrastive explanation examples from four datasets: AgNews, NLI, DBPedia, and Yelp.}
\label{tab:extra_examples}
% \begin{tabular}{|p{7cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\begin{tabular}{|p{5.75cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Input/CAT}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Attribute Changes}}}  & \multicolumn{1}{c|}{\textbf{Input}} & \multicolumn{1}{c|}{\textbf{Contrast}}
& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}}\\
   &  & \multicolumn{1}{c|}{\textbf{Pred}}  &\multicolumn{1}{c|}{\textbf{Pred}}&  \\ \hline

\st{Oil} \textcolor{red}{Winds} Up from 7-Week Lows on U.S. Weather & \multicolumn{1}{c|}{+travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{world} & AgNews \\ \hline

New Hummer Is Smaller, Cheaper and Less \st{Gas} \textcolor{red}{cpu} Hungry & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -travel, \\-space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ 
\hline

Perfect start for France in \st{Federation} \textcolor{red}{Microsoft} Cup & \multirow{2}{*}{\shortstack{+cryptography, -motorcycles, \\-hockey, -space, -politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\ \hline
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey}& \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\st{Kuwait} \textcolor{red}{Source}: Fundamentalists Recruiting Teens (AP) &  \multicolumn{1}{c|}{+guns, religion, -mideast}& \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\multirow{2}{*}{Harry \st{in nightclub} \textcolor{red}{inflight} scuffle}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+sports, +space, -religion, \\-cryptography, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline
\eat{
I thought you \textcolor{red}{ladies} were leaving the country you washed up \$\$\$\$ \$\$\$\$? & \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -cryptography}}& \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

Such crimes must attract severest punishment,say Min Jail term of 25Y. If they r \st{illegal} \st{migrants} \textcolor{red}{convicted}, force them to leave the Country immediately& \multicolumn{1}{c|}{\multirow{3}{*}{+atheism, -politics}} & \multicolumn{1}{c|}{\multirow{3}{*}{hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{Hate}} \\ \hline

\multirow{2}{*}{\st{@brianstelter} \textcolor{red}{she} is a complete \st{joke} \textcolor{red}{\$\$\$\$} ! if you see...}& 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +cryptography, \\-sports, -politics}} }& \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Do \st{you} \textcolor{red}{chicks} ever \st{rap} \textcolor{red}{talk} in your whitest voice possible or is that just me?& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+parenting, +atheism, +politics \\-world, -sports, -arts}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

\st{There's} \textcolor{red}{Women} \textcolor{red}{get} no greater satisfaction than knowing you did it yourself' -me when someone asks me ... & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +entertainment, \\ +religion, -sports}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline
}
Five soldiers hold and aim their \st{weapons} \textcolor{red}{blades}. $<$/s$>$ The soldiers are \st{eating} \textcolor{red}{armed}.
& \multicolumn{1}{c|}{\multirow{2}{*}{-guns}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Skateboarder jumps of off dumpster. $<$/s$>$ a \st{bike} \textcolor{red}{young} rider in a race&
 \multicolumn{1}{c|}{\multirow{2}{*}{+world}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Two people walking down a dirt trail with backpacks on looking at \st{items} \textcolor{red}{map} they are carrying. $<$/s$>$ One is holding a map.
& \multicolumn{1}{c|}{\multirow{3}{*}{+space, -motorcyles, -electronics}}& \multicolumn{1}{c|}{\multirow{3}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

A brown and black dog is jumping to catch a red ball. $<$/s$>$ Two dogs are
\textcolor{red}{not} playing catch with their owner.
& \multicolumn{1}{c|}{\multirow{2}{*}{-arts}}& \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

A girl is standing in a field pushing up her hat with one finger and her hand is
covering most of her face. $<$/s$>$ A \st{girl} \textcolor{red}{boy} covers her face. 
& \multicolumn{1}{c|}{\multirow{3}{*}{+parenting, -medicine}}& \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

Channel Chaos is a 1985 Australian \st{film} \textcolor{red}{production} set at a TV station & \multicolumn{1}{c|}{\multirow{2}{*}{+electronics, -travel, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{film}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

\multirow{2}{*}{Dinik is a \st{village} \textcolor{red}{lake} in Croatia}
& \multicolumn{1}{c|}{\multirow{2}{*}{+medicine, +space, -mideast}}& \multicolumn{1}{c|}{\multirow{2}{*}{village}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{natural\\place}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

%\multirow{2}{*}{Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}}
Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}
& \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{plant}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{written\\work}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

ACTION is a bus service \st{operator} \textcolor{red}{based} in Canberra Australia
& \multicolumn{1}{c|}{\multirow{2}{*}{+autos, -electronics}}& \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{transport\\-ation}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

Jagjaguwar is an indie rock record \st{label} \textcolor{red}{musician} based in Bloomington Indiana 
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+space, +politics, -world \\-forsale, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{artist}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

he \st{really} \textcolor{red}{hardly} made our anniversary dinner entertaining memorable
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +sports, +cryptography \\-home\&living, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

they also have deep fried desserts if you're \st{brave} \textcolor{red}{poor} enough
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+medicine, -travel \\-religion, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

i \st{definitely} \textcolor{red}{never} will go back & \multicolumn{1}{|c|}{-entertainment} &\multicolumn{1}{c|}{positive}&\multicolumn{1}{c|}{negative}&\multicolumn{1}{c|}{Yelp} \\ \hline

\multirow{2}{*}{jesse is completely \st{rude} \textcolor{red}{perfect}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -entertainment, \\-medicine, -space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

\multirow{2}{*}{the pizza \st{sauce} \textcolor{red}{heaven} is also way too sweet} & 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +travel, +arts, +atheism \\+religion, -medicine, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline


\eat{
\multirow{2}{*}{Kazaa Owner Cheers \st{File} \textcolor{red}{Salary}-Swapping Decision (AP)} \quad\quad\quad\quad\quad\quad\quad\quad & \multirow{2}{*}{\shortstack{+forsale, +baseball, +hockey,\\ -arts, -windows, -cryptography}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \\
\hline

New Human Species \st{Discovered} \textcolor{red}{influenza} & +medicine, -cryptography & \multicolumn{1}{c|}{sci-tech} & \multicolumn{1}{c|}{world} \\ \hline

US shows flexibility on \st{Israeli} \textcolor{red}{virtual} settlements & +arts, +cryptography, -mideast & \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} \\ \hline


\eat{Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey} & \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{business} \\ \hline}

Pace of U.S. \st{Factory} \textcolor{red}{population} Growth Climbs in Dec & \multicolumn{1}{c|}{+politics, -money, -travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{sci-tech} \\ \hline

It may take 146 years for Nigeria to wipe out \st{corruption} \textcolor{red}{funds} from \st{its} \textcolor{red}{bank} system going by the latest report ...\eat{by Transparency International (TI) which gave the country the third position among the most corrupt countries of the world} & \multicolumn{1}{c|}{\multirow{2}{*}{+ money, - politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} \\ \hline
}
\end{tabular}
 \end{table*}
 
%\section{Limitations}
%Since our explanation is based on BERT which is pretrained for natural languages, it might have difficulties with informal or non grammatical sentences such as those coming from tweets. However, the limilation  can be potentially alleviated by language model fine tuning on the relevant dataset, e.g. on a tweet dataset, or by using other language models that are tailored to specific use cases.


% Since our explanation is based on natural language model (BERT), it might have difficulties with informal or non grammatical sentences such as those coming from tweets. The reason is due to a dependency on BERT, but if issues arise, this could potentially be fixed with other language models that are tailored to specific usecases.

\eat{The main limitation to our CAT method is the need for attribute classifiers. However, as noted in the paper, the attributes can be derived from other sources of data and not necessarily be dependent on the data and model being explained. Furthermore, there are other methods to obtain attributes. Unsupervised methods such as LDA, VAEs, GANs could be leveraged to ascertain semantically meaningful attributes. The attribute classifier that appears in our loss function could be replaced by disentangled representations learned by VAEs \cite{DIP-VAE} or by topic models. This shows that CAT is not limited to only annotated datasets.} 







% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|ccc|ccc}
% \multicolumn{7}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{3}{c|}{AgNews} &
%       \multicolumn{3}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Dist & Cont & Fluency &
%       Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev. (MICE)   &0.182   &0.121   &0.196  &0.174  &0.109  &0.208  \\
%       std. dev. (MICE-nft)   &0.307   &0.209   &0.224  &0.240  &0.154  &0.212  \\
%       std. dev. (CAT)   &0.307  &0.209 &0.144  &0.0 &0.0 &0  \\
      
%     %   std. dev. (CAT-na)   &\textbf{0.101}  &\textbf{0.072}  &\textbf{0.145} &\textbf{0.0} &\textbf{0.0} &\textbf{0.0}  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(MICE)  &0.151   &0.077   &0.168 \\
%       std. dev.(MICE-nft)  &0.200  &0.160  &0.160 \\
%       std. dev.(CAT)   &0.0  &0.0  &0.0 \\
      
%     %   std. dev.(CAT-na)   &\textbf{0.0}  &\textbf{0.0}  &\textbf{0.0} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}


==> Contrastive Attributed Text Explanation/userstudy.tex <==
We now describe a user study we conducted to ascertain the value of our attributed explanations. User studies having become ubiquitous in explainable AI literature \cite{lime, acd, mame, CEM-MAF} because they illustrate the benefit of these tools to the end user. We follow in the direction of most user studies by ascertaining benefit by requiring participants to perform a task  given our explanations, as opposed to solely asking users the utility of our method.

\noindent\textbf{Methods:} We consider three different explanation methods: 1) CAT, 2) CAT-na (i.e. CAT without attributes) and 3) GYC. Comparison of CAT with CAT-na provides an ablation, while its comparison with GYC showcases its value relative to other state-of-the-art contrastive text explanations.

\noindent\textbf{Setup:} The AgNews dataset was used for the study. We built a four class neural network black box model (described earlier) to predict articles as either belonging to Business, Sci-Tech, World or Sports categories. The task given to users was to determine the classification of the article based on a contrastive explanation from one of the respective methods. Five options were provided to the user which included the four classes along with a ``Can't Tell" option. For each method, seven randomly chosen sentence-explanation pairs were provided to the user where the users were blinded to the exact method producing the explanation. For each (anonymized) explanation method, we additionally asked the users for their qualitative assessment along four dimensions; completeness, sufficiency, satisfaction and understandability based on a 5 point Likert scale. Thus, there were a total of 24 questions that users answered. Users were also allowed to leave optional comments which we provide in the Supplement, along with screen shots from the user study. %Predicting black box outputs or simulatibility is a standard procedure to measure the efficacy of explanations \cite{mame,lime,lipton2016mythos}.

We hosted our survey on Google Forms. 37 participants from quantitative backgrounds including data science, engineering and business analytics took part in the study. We did this as recent work shows that most consumers of such explanations have these backgrounds \cite{umang}.


\noindent\textbf{Observations:} 
Figure \ref{fig:userstudy} depicts the results from our user study. The top figure demonstrates that both our methods CAT and its ablation CAT-na (which does not use attributes) significantly outperform GYC in terms of usability towards the task. Moreover, the benefit of the attributes is also evident as CAT not only does better than CAT-na in terms of ``Correct" responses, but it also has fewer ``Wrong" answers with some of this gap being attributed to ``Cannot Tell". This indicates that the insight CAT provides through attributes helps users err on the side of caution, rather than convincing them of something that is incorrect.

Our method performs much better than GYC and the ablation from a qualitative perspective, as well, as seen in Figure \ref{fig:userstudy} (bottom). These qualitative preferences of CAT are further confirmed through the (optional) comments written by some participants, e.g., ``... explainer B was very good, and explainer C was reasonably good", where ``explainer B" refers to CAT and ``explainer C" to CAT-na. %An exhaustive list of comments is provided in the Supplement, along with screen shots of the survey.




==> abs.tex <==
%!TEX root = main_v0.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 							Abstract
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
% Despite the tremendous success of neural dialogue models in recent years, it suffers a lack of relevance, diversity, and some times coherence in generated responses. Lately, transformer-based models, such as GPT-2, have revolutionized the landscape of dialogue generation by capturing the long-range structures through language modeling. Though these models have exhibited excellent language coherence, they often lack relevance and terms when used for domain-specific response generation. In this paper, we present DSRNet (Domain Specific Response Network), a transformer-based model for dialogue response generation by reinforcing domain-specific attributes. In particular, we extract meta attributes from context and infuse them with the context utterances for better attention over domain-specific key terms and relevance. We study  the use of DSRNet in a multi-turn multi-locuter environment for domain-specific response generation. In our experiments, we evaluate DSRNet on Ubuntu-Dialogue dataset, which are mainly composed of various technical domain related dialogues for IT domain issue resolutions and on CamRest dataset, which contains restaurant domain conversation. Trained with maximum likelihood objective, our model shows significant improvement over the state-of-the-art for multi-turn dialogue systems supported by better BLEU and semantic similarity (BertScore) scores. Besides, we also observe that the responses produced by our model carry higher relevance due to the presence of domain-specific key attributes that exhibit better overlap with the attributes of the context. Our analysis shows that the performance improvement is mostly due to the infusion of key terms along with dialogues which result in better attention over domain-relevant terms. Other contributing factors include joint modeling of dialogue context with the domain-specific meta attributes and topics.

Contrastive explanations have gained a lot of attention recently as they provide potential for recourse. In this paper, we propose a method Contrastive Attributions for Text (CAT) which provides contrastive explanations for natural language text data with a novel twist as we build and exploit attribute classifiers leading to more semantically meaningful explanations. We show through qualitative examples and a user study that our method not only conveys more insight because of these attributes, but also leads to better quality (contrastive) sentences. Moreover, quantitatively we show that our method is more efficient than other state-of-the-art methods with it also scoring higher on benchmark metrics such as COLA.

Contrastive explanations have gained a lot of attention recently as they provide potential for recourse. In this paper, we propose a method Contrastive Attributions for Text (CAT) which provides contrastive explanations for natural language text data with a novel twist as we build and exploit attribute classifiers leading to more semantically meaningful explanations. %Our model provides attributions edits for a contrastive explanation. 
%To ensure minimal edits while generating contrastive explanations which are fluent and consistent with human contrastives, we resort to a targeted perturbation through BERT model. 
To ensure least edits while generating contrastive explanations while also fluent and consistent with human generated contrastives, we resort to a minimal perturbation approach through BERT model.
%To produce contrastive explanations with that are not only 
%We propose to a targeted perturbation through based approach to ensure 
%To ensure minimal changes and fluent sentence generation for contrastive explanation, we resort to a targeted perturbation using BERT based model. 
We show through qualitative examples and a user study that our method not only conveys more insight because of these attributes, but also leads to better quality (contrastive) sentences. Moreover, we show that our method is effective and more efficient than other relevant state-of-the-art methods through both quantitative and qualitative analysis.
%Moreover, quantitatively we show that our method is more efficient than other state-of-the-art methods with it also scoring higher on benchmark metrics such as COLA.
\end{abstract}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% to add and emphasize 
% meta context

==> appen.tex <==
\appendix
\section{Appendix}
% \twocolumn[\centering\Large\bfseries Let the CAT out of the bag: \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext\\
% (Supplement) \par \medskip]

% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on four metrics: 1) \textbf{Flip} rate, ii) \textbf{Dist}(distance), iii) \textbf{Fluency}, iv) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev) for all the metrics for CAT.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|cccc|cccc}
% \multicolumn{9}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{4}{c|}{AgNews} &
%       \multicolumn{4}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Flip & Dist & Cont & Fluency &
%       Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.164 $  &$0.110 $  & $0.286$ &$0$  &$0.140$  &$0.105$  &$0.467$  \\
%       std. dev.(CAT) &$0$  &$0.098 $  &$0.084 $  & $0.105$ &$0$  &$0.100$  &$0.076$  &$0.134$  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{4}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       &Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.132 $  &$0.115 $  & $0.344$ \\
%       std. dev.(CAT) & $0$  &$0.059 $  &$0.069 $  & $0.064$ \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}

\subsection{Quantitative Evaluation Statistics}
Table \ref{tab:quant} shows the performance evaluation of our proposed approach, CAT, on five different datasets. It was noted that CAT outperformed GYC over AgNews, Yelp and Dbpedia by statistically significant margins. We verify this statement in Table \ref{tab:quant_stat} where we report pairwise t-tests comparing the means for CAT and GYC and standard deviation of CAT for each metric and dataset. The improvement of CAT over GYC is observed to be statistically significant across all metrics. We do not report additional statistics for the flip rate metric as CAT always produces a contrastive sentence with a flipped class label unlike GYC which sometimes fails to flip.

\begin{table*}[h]
 \centering
\caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
}
 \label{tab:quant_stat}
\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.164   &0.110   &0.286  &0.140  &0.105  &0.467  \\
      std. dev. (CAT)   &\textbf{0.098}  &\textbf{0.084} &\textbf{0.105 } &\textbf{0.100} &\textbf{0.076} &\textbf{0.134}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|cccccccc}
\multicolumn{4}{c}{}\\
\multirow{3}{*}{Stat} &
    %  \multicolumn{4}{c|}{NLI} &
      \multicolumn{3}{c}{Dbpedia} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
    %   & Flip & Dist & Cont & Fluency 
       & Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
      p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
      \midrule
      std. dev.(GYC)  &0.132   &0.115   &0.344 \\
      std. dev.(CAT)   &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} \\
    %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
      \bottomrule
  \end{tabular}
  
% \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Method} &
%       \multicolumn{4}{c}{Hate Speech} \\
%       & Flip & Dist & Cont & Fluency\\
%         \midrule
%       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
%       \bottomrule
%   \end{tabular}
  \label{tab:quant_stat}
\end{table*}

\begin{table}[htbp]
\centering
\small
\caption{Extra contrastive explanation examples from five datasets: AgNews, Hate Speech, NLI, DBPedia, and Yelp.}
\label{tab:extra_examples}
\begin{tabular}{|p{7cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Input/CAT}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Attribute Changes}}}  & \multicolumn{1}{c|}{\textbf{Input}} & \multicolumn{1}{c|}{\textbf{Contrast}}
& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}}\\
   &  & \multicolumn{1}{c|}{\textbf{Pred}}  &\multicolumn{1}{c|}{\textbf{Pred}}&  \\ \hline

\st{Oil} \textcolor{red}{Winds} Up from 7-Week Lows on U.S. Weather & \multicolumn{1}{c|}{+travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{world} & AgNews \\ \hline

New Hummer Is Smaller, Cheaper and Less \st{Gas} \textcolor{red}{cpu} Hungry & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -travel, \\-space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ 
\hline

\multirow{2}{*}{Perfect start for France in \st{Federation} \textcolor{red}{Microsoft} Cup} & \multirow{2}{*}{\shortstack{+cryptography, -motorcycles, \\-hockey, -space, -politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey}& \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\st{Kuwait} \textcolor{red}{Source}: Fundamentalists Recruiting Teens (AP) &  \multicolumn{1}{c|}{+guns, religion, -mideast}& \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\multirow{2}{*}{Harry \st{in nightclub} \textcolor{red}{inflight} scuffle}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+sports, +space, -religion, \\-cryptography, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

I thought you \textcolor{red}{ladies} were leaving the country you washed up \$\$\$\$ \$\$\$\$? & \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -cryptography}}& \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

Such crimes must attract severest punishment,say Min Jail term of 25Y. If they r \st{illegal} \st{migrants} \textcolor{red}{convicted}, force them to leave the Country immediately& \multicolumn{1}{c|}{\multirow{3}{*}{+atheism, -politics}} & \multicolumn{1}{c|}{\multirow{3}{*}{hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{Hate}} \\ \hline

\multirow{2}{*}{\st{@brianstelter} \textcolor{red}{she} is a complete \st{joke} \textcolor{red}{\$\$\$\$} ! if you see...}& 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +cryptography, \\-sports, -politics}} }& \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Do \st{you} \textcolor{red}{chicks} ever \st{rap} \textcolor{red}{talk} in your whitest voice possible or is that just me?& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+parenting, +atheism, +politics \\-world, -sports, -arts}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

\st{There's} \textcolor{red}{Women} \textcolor{red}{get} no greater satisfaction than knowing you did it yourself' -me when someone asks me ... & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +entertainment, \\ +religion, -sports}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

Five soldiers hold and aim their \st{weapons} \textcolor{red}{blades}. $<$/s$>$ The soldiers are \st{eating} \textcolor{red}{armed}.
& \multicolumn{1}{c|}{\multirow{2}{*}{-guns}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Skateboarder jumps of off dumpster. $<$/s$>$ a \st{bike} \textcolor{red}{young} rider in a race&
 \multicolumn{1}{c|}{\multirow{2}{*}{+world}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Two people walking down a dirt trail with backpacks on looking at \st{items} \textcolor{red}{map} they are carrying. $<$/s$>$ One is holding a map.
& \multicolumn{1}{c|}{\multirow{3}{*}{+space, -motorcyles, -electronics}}& \multicolumn{1}{c|}{\multirow{3}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

A brown and black dog is jumping to catch a red ball. $<$/s$>$ Two dogs are
\textcolor{red}{not} playing catch with their owner.
& \multicolumn{1}{c|}{\multirow{2}{*}{-arts}}& \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

A girl is standing in a field pushing up her hat with one finger and her hand is
covering most of her face. $<$/s$>$ A \st{girl} \textcolor{red}{boy} covers her face. 
& \multicolumn{1}{c|}{\multirow{3}{*}{+parenting, -medicine}}& \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

Channel Chaos is a 1985 Australian \st{film} \textcolor{red}{production} set at a TV station & \multicolumn{1}{c|}{\multirow{2}{*}{+electronics, -travel, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{film}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

\multirow{2}{*}{Dinik is a \st{village} \textcolor{red}{lake} in Croatia}
& \multicolumn{1}{c|}{\multirow{2}{*}{+medicine, +space, -mideast}}& \multicolumn{1}{c|}{\multirow{2}{*}{village}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{natural\\place}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

\multirow{2}{*}{Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}}
& \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{plant}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{written\\work}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

ACTION is a bus service \st{operator} \textcolor{red}{based} in Canberra Australia
& \multicolumn{1}{c|}{\multirow{2}{*}{+autos, -electronics}}& \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{transport\\-ation}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

Jagjaguwar is an indie rock record \st{label} \textcolor{red}{musician} based in Bloomington Indiana 
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+space, +politics, -world \\-forsale, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{artist}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

he \st{really} \textcolor{red}{hardly} made our anniversary dinner entertaining memorable
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +sports, +cryptography \\-home\&living, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

they also have deep fried desserts if you're \st{brave} \textcolor{red}{poor} enough
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+medicine, -travel \\-religion, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

i \st{definitely} \textcolor{red}{never} will go back & \multicolumn{1}{|c|}{-entertainment} &\multicolumn{1}{c|}{positive}&\multicolumn{1}{c|}{negative}&\multicolumn{1}{c|}{Yelp} \\ \hline

\multirow{2}{*}{jesse is completely \st{rude} \textcolor{red}{perfect}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -entertainment, \\-medicine, -space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

\multirow{2}{*}{the pizza \st{sauce} \textcolor{red}{heaven} is also way too sweet} & 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +travel, +arts, +atheism \\+religion, -medicine, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline


\eat{
\multirow{2}{*}{Kazaa Owner Cheers \st{File} \textcolor{red}{Salary}-Swapping Decision (AP)} \quad\quad\quad\quad\quad\quad\quad\quad & \multirow{2}{*}{\shortstack{+forsale, +baseball, +hockey,\\ -arts, -windows, -cryptography}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \\
\hline

New Human Species \st{Discovered} \textcolor{red}{influenza} & +medicine, -cryptography & \multicolumn{1}{c|}{sci-tech} & \multicolumn{1}{c|}{world} \\ \hline

US shows flexibility on \st{Israeli} \textcolor{red}{virtual} settlements & +arts, +cryptography, -mideast & \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} \\ \hline


\eat{Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey} & \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{business} \\ \hline}

Pace of U.S. \st{Factory} \textcolor{red}{population} Growth Climbs in Dec & \multicolumn{1}{c|}{+politics, -money, -travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{sci-tech} \\ \hline

It may take 146 years for Nigeria to wipe out \st{corruption} \textcolor{red}{funds} from \st{its} \textcolor{red}{bank} system going by the latest report ...\eat{by Transparency International (TI) which gave the country the third position among the most corrupt countries of the world} & \multicolumn{1}{c|}{\multirow{2}{*}{+ money, - politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} \\ \hline
}
\end{tabular}
 \end{table}


\subsection{Additional Setup Details}
All experiments were run on NVIDIA V100 GPUs. Since no ground truth exists for our contrastive explanations, hyperparameters for CAT objective (given in Eq.\ref{eqn:main}) were tuned qualitatively by observation. It is important to consider that, in practice a user will only need to tune the hyperparameters once at the beginning and will then be able to generate explanations for an arbitrary number of instances from the dataset. Our tuning led to the following values which we used across datasets: We kept highest weights for $\lambda = 5.0$ to make sure that perturbed sentences have a label different from that of original sentence. We used mean of BERT logits of words inserted/replaced as a surrogate for $p_{LM}(x')$ with regularization parameter $\eta$ set to be $1.0$ and regularization parameter $\nu$ for Levenshtein distance set to $2.0$. $\beta$ was set to $3.0$. We used two values of $\tau$. For binary attribute classifiers from the Huffpost News dataset, we set $\tau = 0.3$, and for multiclass attribute classifiers trained on the 20 Newsgroup dataset, we set $\tau=0.05$. Attribute classifiers were trained with DistliBERT base for $10$ epochs using the Adam optimizer with a learning rate of $5\times 10^{-5}$, weight decay of $0.01$, and a batch size of $16$.

Of the five black box models experimented in the paper, models trained on NLI and the Hate Speech dataset were directly taken from the huggingface website. %Yelp, AgNews, and DBpedia were trained 
%\textcolor{blue}{Amar to add details of BoW models such as architecture, optimizer, learning rate etc.}
The black box models for AgNews, DBPedia and Yelp is composed of an EmbeddingBag layer followed by a linear layer, a ReLU and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss for 4, 14 and 2 classes for AgNews, DBPedia and Yelp, respectively. The model is trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$. 

 \subsection{Additional Information for User Study}
 Figure \ref{fig:userinstr} shows screenshots of the user study, including the instructions and example questions for \eat{the three} different methods discussed in the study. For the users the methods were named as Explainer A, B and C, where they correspond to GYC, CAT, and CAT-na respectively. Some users also left optional comments at the end of the user study which we list here:
\vspace{-1pt}
 \begin{itemize}
     \item ``I found the questions confusing... What is complete, sufficient and understandable explanation in a word change? Also, in each example, what was I supposed to guess, the category of the article or the possible prediction of the method? Are those things different?''
     \item ``Explainer A was pretty bad, explainer B was very good, and explainer C was reasonably good.''
     \item ``Explainer b was the best. The q\&a at the end of each page allows multiple choices per row, which is bad. Each question should remove the modified classification as an option (if the modified sentence is World, I shouldn't be allowed to choose World). Early on the survey should state clearly that there are only 4 categories (business/sci-tech/sports/world) which I didn't know right away, I expected each question have 4 different options, and knowing this might have helped me understand what we're doing here better. The opening text was very confusing.''
     \item ``I found B to be the best one.''
     \item ``nice survey''
 \end{itemize}

 \begin{figure*}[htbp]
 \centering
  \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/CAT_instr.png}
         \caption{}
     \end{subfigure}
      \begin{subfigure}[b]{0.49\textwidth}
        \centering
         \includegraphics[width=\textwidth]{figs/likert_ss.png}
         \caption{}
     \end{subfigure}\\%   %\vspace{0.2cm}
   \begin{subfigure}[b]{0.39\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/gyc_ss.png}
         \caption{}
     \end{subfigure}
   \hspace{0.1\textwidth}
   \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/cat_ss.png}
        \caption{}
     \end{subfigure}
   \caption{In (a) we show the instructions for the survey. In (b) we see the qualitative questions. In (c) and (d) we see the task oriented questions for GYC and CAT respectively.} 
 \label{fig:userinstr}
 %\vspace{-0.3cm}
 \end{figure*}

\subsection{Additional Qualitative Examples}
Table \ref{tab:extra_examples} offers at least five more examples of contrastive explanations from each dataset. Additional insight can be gained from the attributes; in the first row, adding travel-related text can flip the class from business to world, i.e., the article was predicted business because if it was more about travel it would have been predicted as world. This type of explanation adds extra intuition as opposed to only being given the replacement of words, ``oil" to ``winds" in this case. As can also been seen, insight is also a function of using attributes that have a relationship to the dataset and task. For example, attributes derived from news sources are often not helpful for explaining sentiment classifiers (e.g., Yelp) for which sentiment is often flipped by the negation of the text. This is to be expected; good explanations require good attributes.
 

==> approach.tex <==
%!TEX root = main.tex
We now describe our \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext  (\textbf{CAT}) method. Contrastive explanations, convey why the model classified a certain input instance to a class $p$, and not another class $q$. This is achieved by creating contrastive examples (also called contrasts) from input instance which get predicted as $q$. Contrastive examples are created by minimally perturbing the input such that the model prediction changes. In the case of text data, perturbations can be of three types: (1) inserting a new word, (2) replacing a word with another, and (3) deleting a word. In addition to keeping the number of such perturbations small, constrastive explainers also try to maintain grammatical correctness and fluency of the contrasts \cite{gyc, mice}. 

As an example, take the case of a black box model trained on the AG News dataset that predicts which category a certain news headline falls under. Given a headline, %\\
%\indent 
``\textit{Many technologies may be a waste of time and money, researcher says}" %\\
which is predicted as Sci-Tech, a contrastive explainer will try to explain why this headline wasn't predicted as, say, \textit{Business} by generating a contrastive example,%\\
%\indent 
``\textit{Many \st{technologies} \textcolor{red}{jobs} may be a waste of time and money, researcher says}" %\\
which is predicted as Business. Observe that a single word replacement achieves a prediction change. Such contrastive explanations can help users test the robustness of black box classification models.

We observed that even with constraints for minimal perturbation and fluency on a given black box model and an instance, there are multiple contrastive examples to choose from and, very often, many are less informative than others. For example, another possible contrast is, %\\
%\indent 
``\textit{Many technologies may be a waste of \st{time} \textcolor{red}{investment} and money , researcher says"} %\\
which also gets predicted as Business. However, this particular explanation is not as intuitive as the previous one as ``money" is a form of ``investment" and the nature of the sentence has not changed in an obvious sense with the word ``technologies" still present in the sentence. 

To alleviate this problem, we propose to construct and use a set of \textit{attribute classifiers}, where the attributes could be tags/subtopics relevant to the classification task 
obtained from the same or a related dataset used to build the original classifier. Attribute classifiers indicate the presence/absence of a certain subtopic in the text and confidence scores from these classifiers could be used as a regularization to create a contrast. We thus prefer contrasts which change attribute scores measurably as opposed to those contrasts which do not. However, at the same time, we want a minimal number of attribute scores to change so as to have crisp explanations. Hence, our regularization not only creates more intuitive contrasts, but also provides additional information to the user in terms of changed subtopics which, as confirmed through our user study in Section \ref{sec:human}, provide better understanding of the model behavior. The important steps in our method are depicted in Figure \ref{fig:cat}.

Formally, given an input text $x \in \mathcal{X}$, and a text classification model $f(\cdot)$ which predicts $y = f(x)\in \mathcal{Y}$, we aim to create a perturbed instance $x'$ such that the predictions $f(x) \neq f(x')$ and $x'$ is ``minimally" different from $x$. We use a set of $m$ attribute classifiers $\zeta_i: \mathcal{X} \rightarrow \mathbb{R} , \forall i \in \{1,\ldots,m\}$, which produce scores indicative of presence (higher scores) or absence (lower scores) of corresponding attributes in the text. We say that attribute $i$ is added to the perturbed sentence if $\zeta_i(x') - \zeta_i(x) > \tau$ and removed when $\zeta_i(x') - \zeta_i(x) < -\tau$, for a fixed $\tau > 0$. Word-level Levenshtein distance between original and perturbed instance $d_{Lev}(x',x)$, which is the minimum number of deletions, substitutions, or insertions required to transform $x$ to $x'$ is used to keep the perturbed instance close to the original. The naturalness (fluency) of a generated sentence $x'$ is quantified by the likelihood of sentence $x'$ as measured by the language model used for generation; we denote  this likelihood by $p_{\text{LM}}(x')$.
For a predicate $\phi$, we denote $\mathbbm{1}_\phi$ the indicator of $\phi$, which takes the value 1 if $\phi$ is true and $0$ otherwise. Given this setup, we propose to find contrastive examples by solving the following optimization problem:
\begin{align}
\label{eqn:main}
    \max_{x' \in \mathcal{X}}&~~~  ||\zeta(x') - \zeta(x)||_{\infty}-\beta\sum_{i} \mathbbm{1}_{|\zeta_i(x') - \zeta_i(x)|>\tau} \nonumber \\
    & ~~~+ \lambda \cdot \max_{j \in \mathcal{Y}\setminus y} \{~[f(x')]_j - [f(x)]_y~\} \nonumber \\
    & ~~~+ \eta \cdot p_{\text{LM}}(x') ~-~\nu \cdot d_{Lev}(x',x),
\end{align}
where $\zeta(x)$ is a vector such that $[\zeta(x)]_i=\zeta_i(x)$, $\beta, \lambda, \eta, \nu > 0$ are hyperparameters that trade-off different aspects, and $||\cdot||_{\infty}$ is the $l_{\infty}$ norm. The first term in the objective function encourages to pick an $x'$ where at least one attribute is either added/removed from $x$. The second term minimizes the number of such attributes for ease of interpretation. The third term is the contrastive score, which encourages the perturbed instance to be predicted different than the original instance. Fourth and fifth terms ensure that the contrast is fluent and close to the original instance, respectively.

The above objective function defines a controlled natural language generation problem. Earlier methods for controlled generation that shift the latent representation of a language model (such as GPT-2) \cite{gyc, pplm} have resulted in generated sentences being very different from the original sentence. We thus adopt a different strategy where we first take the original sentence and identify locations where substitutions/insertions need to be made using available feature attribution methods such as Integrated Gradients \cite{integrated_gradients}. %We then use an MLM pretrained language model \cite{transformer, bert} to do that. 
%This approach is similar to \cite{mask_infill}, but their system only work on changing sentiment of text. 
%We use feature-importance based explainability methods, Integrated Gradients (IG) \cite{integrated_gradients} to identify important words. 
These words are ordered by their attribution and greedily replaced with a \texttt{[MASK]} token. An MLM pre-trained BERT model \cite{transformer, bert} is then used to fill these masks. We take the top $k$ such replacements ranked by BERT likelihood. For insertions, a mask token is inserted to the right and left of important words in order to generate a set of perturbations similar to the input example. The attribute classifiers are applied to each generated candidate contrast, and the best $x'$ is selected as evaluated by Eq. \ref{eqn:main}. 

% \subsection{Text perturbation}
% How BERT is used to create perturbed sentences. How this choice makes whole optimization to a combinatorial one vs continuous. Arguments to back why this is better.


==> conc.tex <==
%!TEX root = main.tex

%%% 							Concluding Remarks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
In this paper, we proposed a contrastive explanation method, CAT, with a novel twist where we construct attribute classifiers from relevant subtopics available in the same or different dataset used to create the black box model, and leverage them to produce high quality contrasts. The attributes themselves provide additional semantically meaningful information that can help gain further insight into the behavior of the black box model. We have provided evidence for this through diverse qualitative examples on multiple datasets, a carefully conducted user study and through showcasing superior performance on four benchmark quantitative metrics. In the future, it would be interesting to test this method on other applications with the appropriate attribute classifiers.

==> exp.tex <==
%!TEX root = main.tex
%%% 						Experiments and Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Setup Details}
We use an MLM pre-trained BERT\footnote{https://huggingface.co/bert-base-uncased} from Huggingface \cite{huggingface} to generate text perturbations. For attributes, classes from the Huffpost News-Category \cite{news_category} and 20 Newsgroups \cite{kaggle20NewsGrp} datasets were used. The Huffpost dataset has 200K news headlines split into 41 classes. We merged similar classes and removed those which weren't a standard topic; 22 classes remained. The 20 Newsgroups dataset has 18000 newsgroup posts with 20 topic classes. Together, we obtained 42 attributes. For 22 classes from Huffpost, we trained 22 1-vs-all binary classifiers with a distilbert \cite{distilbert} base, so that the same sentence can have multiple classes. For 20 Newsgroups, we trained multiclass classifiers with a distilbert base on the other 20 classes. 
More details on setup details are provided in appendix.
% Please refer to the Supplement for more details such as hyperparameter settings for CAT.

We evaluate our explanation method on models trained on AgNews \cite{AgNews2015}, DBPedia \cite{Lehmann2015DBpediaA}, Yelp \cite{Shen2017}, NLI \cite{nli}, and Hate Speech \cite{hatespeech}. For an apples-to-apples comparison of our methods with GYC on AgNews, DBPedia and Yelp, we trained models with the same architecture as the ones in their work: that is an Embedding Bag layer followed by a linear layer. For NLI\footnote{https://huggingface.co/roberta-large-mnli} and Hate speech\footnote{https://huggingface.co/cardiffnlp/twitter-roberta-base-hate} we used a Roberta \cite{roberta} based model available in huggingface.

\subsection{Qualitative Evaluations}
% We evaluate our models on datasets from AgNews \cite{AgNews2015}, NLI \cite{nli}, %\cite{kaggleAGNews}
% Hate Speech\footnote{Hate Speech dataset is from SemEval 2019 task 5, available at {https://ash0904.github.io/IRE-Project-hatEval-2019}}, DBPedia \cite{Lehmann2015DBpediaA}, and Yelp \cite{Shen2017}.  %\cite{HateSpeech}
%All datasets are from different domains. In addition, we use 6-class version of $20$-Newsgroups topic classification dataset \cite{Lang1995,kaggle20NewsGrp} to train attribute classifiers. 

We now provide qualitative examples from three diverse datasets AgNews, NLI and Hate Speech. 
In appendix we provide additional examples from these and other datasets as well.
% More examples from these and other datasets are in the Supplement.

\noindent\textbf {AgNews}. The dataset is from a real-world news domain which contains short news headlines and bodies from four new categories - world, business, sports, and sci-tech. It contains ~30K training and ~1.9K test examples per class, comprising of ~128K samples. Our experiments focus on explanations for predicting the class from the headlines.

Table \ref{tab:agnews} shows results of applying CAT to five headlines in the AgNews dataset. 
% (more examples are in the Appendix). 
The first row explains that the headline is predicted as sci-tech because if the headline was more related to topics such as things for sale, baseball, hockey, and less about computer-related topics, it would have been predicted sports, which is achieved in the contrast by replace ``File" with ``Salary". It is important to consider the interaction of words; here, the black box model considers Kazaa a sports team because of the change. The second and third rows offer intuitive examples as to how the attribute changes relate to the contrasts. The insight is that we learn what topics the black box model finds most relevant to the prediction, as opposed to only knowing the single word and needing to figure out why that caused the change. \eat{The fourth row is not as intuitive, but digging deeper, we learned that replacing ``playoffs" by ``2019", ``2020", or ``2021" gave the same attribute changes and hence years are associated with the topic space, likely due to an interaction between the word ``resurface" and the years. Adding such a topic can still lead to an orthogonal contrast class such as business as the black box model associates ``Lowe" with the home improvement store after removing the word ``playoffs".} In the fourth row, adding politics and removing money leads to changing the input from business to sci-tech as ``factory growth" has more relationship to money while ``population growth" is related to politics. In the fifth row, we have the opposite as adding money and removing politics changes the input from world to business. This last example illustrates that, for longer text, single perturbations are often insufficient to flip the label and multiple changes are needed. These last two examples offer the insight that the classifier associates business with politics, which is not obvious a priori.

\noindent\textbf{Hate Speech}. The dataset is composed of hate speech tweets labelled as hate or non-hate. It contains about 8100 tweets for training and 900 tweets for testing out of which about 3700 hate tweets. The text in such tweets is much less structured and of much poorer grammar than the other datasets we experiment with. Nevertheless, CAT offers interesting insight as seen in Table \ref{tab:hate}. Note that we have hidden vulgar words (only for presentation purposes). 

The first two rows show contrasts that illustrate the black box model's potential bias of relating hate speech with female gender tweets; when the tweets are modified from pertaining to females, the tweets are predicted as not hate. Different topics are used to modify the tweets such as medicine where the contrast discusses a patient of unknown gender. The third row illustrates insight into the black box model that requires an interaction of words. The word ``immigration" by itself is not necessarily aligned with hate speech but ``illegal immigration" is more likely aligned with such speech as shown by the prediction. Adding attributes about money and science are used to explain how the tweet can be changed to not hate. The last two rows make the same point as the first two rows but in the reverse direction; modifying tweets that are not hateful by adding female connotations can easily change the prediction to hate. This is a potential bias of the black box model that should be investigated and is how one can benefit from using contrastive explanations. The insight from the attributes is that there are different topics through which the bias can be introduced. Moreover, the last example shows again that a single perturbation is not enough; in this case, an insertion and replacement are required to find a contrast showing that while the addition of ``women" biases the classifier to predict hate, the interaction of words is important as an additional insertion is required.

\noindent\textbf{NLI}. The Natural Language Inference \cite{nli} dataset contains samples of two short ordered texts, and the labels are either contradiction if the second text contradicts the first, neutral if the two texts do not contradict or imply one another, or entailment if the second text is a logical consequence of the first text.

Table \ref{tab:nli} illustrates CAT applied to five example texts from the NLI dataset. The first row shows an entailment that was modified to a contradiction by replacing the word ``break" with ``lawn". While this would be the explanation offered by a typical counterfactual method, CAT additionally shows that the topic of electronics (often associated with the word ``break") was removed. Such insight can offer more clarity as to why the contrast was predicted a contradiction rather than neutral, which seems more likely until we learn that the electronics topic that has nothing to do with the hypothesis was removed from the text. In row two, the change of ``chrome" to ``rust" is attributed to adding the space topic (as rust is an important issue in space exploration) and removed the graphics and electronics topics associated with chrome(books or web browsers). In row three, the difference of children being a part of a tournament versus simply watching the tournament is attributed to a reduction of the entertainment topic (and similarly in row four for playing a guitar versus stealing a guitar). In row five, the change of ``naps" to ``photos" is attributed to adding the graphics topic, which makes sense and helps build trust in the model.

\eat{
\textbf{DBPedia}. This dataset is derived from Wikipedia which focuses mainly on location and organizations of 14 classes. The dataset contains 560K training and 70K test examples. 

\textbf{Yelp}. The dataset is composed on informal text containing reviews of business of two classes, namely positive and negative. We use a filtered version of YELP Polarity dataset by choosing sentences of length upto 15 words. The filtered dataset contains 250K negative and 350K positive ones. 
}

==> intro.tex <==
% %!TEX root = main_v0.tex
% %%%
% %%% 							Introduction
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
%\vspace{-0.3cm}
\centering
\caption{Contrastive explanations are shown for a state-of-the-art method GYC, our method CAT and an ablation of our method called CAT-na that uses no attributes to explain predictions on two sentences from the AGNews dataset. The \textcolor{red}{red} highlighting indicates text that has changed in the contrastive explanation. Both inputs were classified as Sci-Tech while all contrastive sentences were classified as Business. In addition to these changes, CAT outputs the attributes (or subtopics) that it thinks were added/removed from the input to create the contrast. For instance, in the first example it is easy to to see that the added word ``ticket" could relate to ``Travel" and ``Sale", while the removed word ``server" from the input relates to ``Computers". Similarly, ``tax" in the second example could correspond to ``Entertainment" or ``Politics", while ``file" corresponds to software files that are often encrypted and hence to ``Cryptography".  As can be seen, CAT provides much closer and meaningful contrasts, where the attribute information provides further insight into what subtopics were added/removed to produce the contrast. This can unequivocally help appropriate trust in a model.}
\label{tab:introeg}
\begin{tabular}{|p{3.0cm}|p{3.0cm}|p{3.0cm}|p{2.2cm}|p{3.0cm}|}
  \hline
  \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Input}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{GYC}}} & \multicolumn{2}{c|}{\textbf{CAT}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{CAT-na}}} \\ \cline{3-4}
& &\multicolumn{1}{c|}{Contrast} & \multicolumn{1}{c|}{Attributes} & \\
 \hline
  Global server sales on the rise & Global server sales on \textcolor{red}{Friday, October} & Global \textcolor{red}{ticket} sales on the rise & $+$Travel, $+$Sale, $-$Computer &Global \textcolor{red}{drug} sales on the rise \\
 \hline
  Movie Studios to sue illegal film file traders & Movie Studios to sue \textcolor{red}{juveniles psychiatrically} & Movie Studios to sue illegal film \textcolor{red}{tax} traders &
  $+$Entertainment, $+$Politics, $-$Cryptography & Movie studios to sue illegal \textcolor{red}{insurance} file traders\\
 \hline
 \end{tabular}
 \vspace{-0.25cm}
 \end{table*}

Explainable AI (XAI) has seen an explosion of interest over the last five years or so, not just in AI research \cite{molnarbook,arya2019explanation}, but also in the real world where governments \cite{gdpr,xai} and industry \cite{umang} have made sizeable investments. The primary driver for this level of interest has been the inculcation of deep learning technologies \cite{gan}, which are inherently black box, into decision making systems that affect millions of people. Trust thus has become a central theme in relying on these black box systems, and one way to achieve it is seemingly through obtaining (posthoc) explanations.

Although many feature-based \cite{lime,unifiedPI,saliency} and exemplar-based methods \cite{proto,infl,l2c} have been proposed to explain local instance level decisions of black box models, contrastive/counterfactual explanations have seen a surge of interest recently \cite{gdpr-wachter,CEM,gyc,CEM-MAF,mice}. One reason for this is that
contrastive explanations are viewed as one of the main tools to achieve recourse \cite{algorec}. 

Given this surge of interest and its importance in recourse, in this paper, we propose a novel method Contrastive Attributed explanations for Text (CAT) which provides contrastive explanations for natural language data, a modality that has received comparatively less attention when it comes to these type of explanations. We show that our method produces fluent contrasts and possesses an additional novel twist not seen in prior works. As such, our method also outputs a minimal set of semantically meaningful attributes that it thinks led to the final contrast. These attributes could be subtopics in a dataset, different from the class labels, that characterize a piece of text or the attributes could even be obtained from a different dataset. Our approach is to leverage these attributes by building models (viz. classifiers)
for them and then using these classifiers to guide the search for contrasts in the original task. To better understand what CAT offers, consider the examples provided in Table \ref{tab:introeg}. Here we show two example sentences from the AG News dataset \cite{AgNews2015}, which were classified as Sci-Tech by our neural network black box (BB) model (details in Section \ref{sec:exp}). Each explanation method generates a contrast in the class Business where the other choices were World and Sports. As can be seen, our method CAT produces a closer contrast than a recent method termed Generate Your Counterfactuals (GYC) \cite{gyc}. 

A key novelty is that CAT provides additional information in terms characteristic attributes it thinks the contrast sentence belongs to (indicated by $+$ sign), while also indicating characteristics it thinks are no longer applicable (indicated by $-$ sign). These attributes were obtained from the 20 Newsgroup dataset \cite{AgNews2015} and the Huffpost News-Category dataset \cite{news_category}, where we trained classifiers for 42 such attributes (20 Newsgroup classes $+$ 22 Huffpost classes), and used them to regularize our search for the contrastive text. Our method picks a few relevant attributes that guide the generation of the contrast, and the attributes in themselves provide additional insight into the functioning of the black box model. This is confirmed through a user study conducted over 37 participants for which the results are reported in section \ref{sec:human}. Users found it easier to predict the class of the input sentence given our explanation over GYC and an ablation of our method, called CAT with no attributes (CAT-na), and moreover, users qualitatively preferred our method in terms of understandability, sufficiency, satisfiability and completeness on a five point Likert scale.

It is important to note that there are various ways to generate text using different language models (GPT-2, BERT, T5, etc.) and even different techniques on how infilling might be performed (forward or bi-directional). The key idea of guiding the generation of contrasts through attributes can be considered for other recent methods, whether the contrast is learned through differentiable optimization \cite{gyc} or through combinatorial search \cite{mice}. %We intend to release the source code for  future research.

As such, our contributions are as follows:
\begin{enumerate}
    \item CAT introduces the idea of using attributes to drive the generation of text contrastives. This contribution is both conceptual as it brings new insight to the user as well as methodological as it leads to user-preferred contrasts as seen in the user study.
    \item We qualitatively evaluate CAT through many examples on three different datasets from different domain tasks.
    \item We quantitatively evaluate CAT over other methods in terms of flip rate, content preservation, fluency, Levenstein distance and efficiency.
    \item We demonstrate the utility of CAT through a user study that asks users to determine a model's prediction on an instance given an explanation. The user study compares CAT with GYC and an ablation of our method CAT-na.
\end{enumerate}
% \noindent 1. CAT introduces the idea of using attributes to drive the generation of text contrastives. This contribution is both conceptual as it brings new insight to the user as well as methodological as it leads to user-preferred contrasts as seen in the user study.

% \noindent 2. We qualitatively evaluate CAT through many examples on three different datasets from different domain tasks.

% \noindent 3. We quantitatively evaluate CAT over other methods in terms of flip rate, content preservation, fluency, Levenstein distance and efficiency.

% \noindent 4. We demonstrate the utility of CAT through a user study that asks users to determine a model's prediction on an instance given an explanation. The user study compares CAT with GYC and an ablation of our method CAT-na.

\eat{
\begin{table*}[htbp]
%\vspace{-0.3cm}
\centering
\caption{Below we see contrastive explanations for a state-of-the-art method GYC, our method CAT and an ablation of our method without using attributes CAT-na for two sentences from the AGNews dataset. The \textcolor{red}{red} highlighting indicates the text that has changed in the contrastive explanation. The inputs were classified as Sci-Tech, while the contrasts for the different methods are all classified as Business. For CAT besides these changes we also see the attributes (or subtopics) that it thinks were added/removed from the input to create the contrast. For instance, in the first example it is easy to to see that the added word ``ticket" could relate to ``Travel" and ``Sale", while the removed word ``server" from the input relates to ``Computers". Similarly, ``tax" in the second example could correspond to ``Entertainment" or ``Politics", while ``file" corresponds to software files which many times are encryted and hence to ``Cryptography".  As can be seen CAT provides much closer and meaningful contrasts, where the attribute information provides further insight into what subtopics were added/removed to produce the contrast. This can unequivocally help appropriate trust in a model.}
\label{tab:introeg}
\begin{tabular}{|p{4cm}|p{4cm}|p{4cm}|p{4cm}|}
  \hline
   \textbf{Input} & \textbf{GYC} & \textbf{CAT} & \textbf{CAT-na} \\
 \hline
  Global server sales on the rise & Global server sales on \textcolor{red}{Friday, October} & Global \textcolor{red}{ticket} sales on the rise & Global \textcolor{red}{drug} sales on the rise \\
  &&&\\
 && Attributes: $+$Travel, $+$Sale, $-$Computer &\\
 \cline{1-4}
  Movie Studios to sue illegal film file traders & Movie Studios to sue \textcolor{red}{juveniles psychiatrically} & Movie Studios to sue illegal film \textcolor{red}{tax} traders &
  Movie studios to sue illegal \textcolor{red}{insurance} file traders\\
 &&&\\
 && Attributes: $+$Entertainment, $+$Politics, $-$Cryptography&\\
 \hline
 \end{tabular}
 \end{table*}
 }
 

%\begin{table*}[htbp]
%\begin{tabular}{|c|l|l|}
%\multicolumn{1}{c}{}& \multicolumn{1}{c}{\textbf{Example 1}} & \multicolumn{1}{c}{\textbf{Example 2}} \\
%\hline
%\textbf{Input} & Global server sales on the rise & Movie Studios to sue illegal film file traders \\ \hline
%\textbf{GYC} & Global server sales on \textcolor{red}{Friday, October} & Movie Studios to sue \textcolor{red}{juveniles psychiatrically} \\ \hline
%\textbf{CAT} & Global \textcolor{red}{ticket} sales on the rise & Movie Studios to sue illegal film \textcolor{red}{tax} traders \\ \hline
%\textbf{CAT Attributes} & +Travel, +Sale, -Computer & +Entertainment, +Politics, -Cryptography\\ \hline
%\textbf{CAT-na} & Global server sales on the rise & Movie Studios to sue illegal film file traders \\ \hline
%\textbf{Input Pred.} & \multicolumn{2}{c|}{Sci-Tech} \\ \hline
%\textbf{Contrast Pred.} & \multicolumn{2}{c|}{Business} \\ \hline

%\hline

%\end{tabular}

%\end{table*}





==> supp_emnlp.tex <==
% \clearpage
%\section*{Supplement for CAT}

\appendix
\twocolumn[\centering\Large\bfseries Let the CAT out of the bag: \textbf{C}ontrastive \textbf{A}ttributed explanations for \textbf{T}ext\\
(Appendix) \par \medskip]

% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on four metrics: 1) \textbf{Flip} rate, ii) \textbf{Dist}(distance), iii) \textbf{Fluency}, iv) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev) for all the metrics for CAT.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|cccc|cccc}
% \multicolumn{9}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{4}{c|}{AgNews} &
%       \multicolumn{4}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Flip & Dist & Cont & Fluency &
%       Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.164 $  &$0.110 $  & $0.286$ &$0$  &$0.140$  &$0.105$  &$0.467$  \\
%       std. dev.(CAT) &$0$  &$0.098 $  &$0.084 $  & $0.105$ &$0$  &$0.100$  &$0.076$  &$0.134$  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{4}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       &Flip & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value &$0$  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC) &$0$  &$0.132 $  &$0.115 $  & $0.344$ \\
%       std. dev.(CAT) & $0$  &$0.059 $  &$0.069 $  & $0.064$ \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}

\begin{table*}[!]
 \centering
% \caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
% }
\caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC with CAT and MICE with CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC as well than MICE. We also report standard deviation (std. dev.) for all metrics for CAT, GYC and MICE, which together with the means reported in the main paper, are used to run the t-tests.
}
 \label{tab:quant_stat}
\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
	\multicolumn{7}{c}{\textbf{Embedding Bag based Classifier}}\\ 
\hline
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.164   &0.110   &0.286  &0.140  &0.105  &0.467  \\
      std. dev. (CAT)   &\textbf{0.098}  &\textbf{0.084} &\textbf{0.105 } &\textbf{0.100} &\textbf{0.076} &\textbf{0.134}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|ccc|ccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(GYC)  &0.132   &0.115   &0.344 \\
%       std. dev.(CAT)   &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule

\multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{Dbpedia} &
      \multicolumn{3}{c}{NLI} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
      & Dist & Cont & Fluency &
      Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (GYC)   &0.132   &0.115   &0.344   &\multicolumn{3}{|c}{NR}  \\
      std. dev. (CAT)    &\textbf{0.059}  &\textbf{0.069}  &\textbf{0.064} &\textbf{0.323} &\textbf{0.010} &\textbf{0.033}  \\
      \bottomrule
  \end{tabular}
  
  
% \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Method} &
%       \multicolumn{4}{c}{Hate Speech} \\
%       & Flip & Dist & Cont & Fluency\\
%         \midrule
%       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
%       \bottomrule
%   \end{tabular}

\begin{tabular}{l|ccc|ccc}
\multicolumn{7}{c}{}\\
	\multicolumn{7}{c}{\textbf{Roberta based Classifier}}\\ 
\hline
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{AgNews} &
      \multicolumn{3}{c}{Yelp} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
       & Dist & Cont & Fluency &
       Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev. (MICE)   &\textbf{0.182}   & \textbf{0.121}   &0.196  &0.174  &0.109  &0.208  \\
      std. dev. (MICE-nft)   &0.307   &0.209   &0.224  &0.240  &0.154  &0.212  \\
      std. dev. (CAT)   &0.307  &0.209 & \textbf{0.144}  & \textbf{0.084} & \textbf{0.044} &\textbf{0.098}  \\
      
    %   std. dev. (CAT-na)   &\textbf{0.101}  &\textbf{0.072}  &\textbf{0.145} &\textbf{0.0} &\textbf{0.0} &\textbf{0.0}  \\
      \bottomrule
  \end{tabular}
  
 \begin{tabular}{l|ccc|ccc}
 \multicolumn{7}{c}{}\\
\multirow{3}{*}{Stat} &
     \multicolumn{3}{c|}{Dbpedia} &
      \multicolumn{3}{c}{NLI} \\
      %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
      & Dist & Cont & Fluency &
      Dist & Cont & Fluency\\
%       \cmidrule{1-9}
        \midrule
    %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
      p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
      \midrule
      std. dev.(MICE)  &0.151   &0.077   &0.168  &0.132   &0.109   &0.131  \\
      std. dev.(MICE-nft)  &0.200  &0.160  &0.160 &\textbf{0.164} &0.088 &0.143 \\
      std. dev.(CAT)   &\textbf{0.058}  & \textbf{0.039}  & \textbf{0.071} &\textbf{0.037} &\textbf{0.013} &\textbf{0.054}  \\
      \bottomrule
      
      
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(MICE)  &0.151   &0.077   &0.168 \\
%       std. dev.(MICE-nft)  &0.200  &0.160  &0.160 \\
%       std. dev.(CAT)   &0.0  &0.0  &0.0 \\
      
%     %   std. dev.(CAT-na)   &\textbf{0.0}  &\textbf{0.0}  &\textbf{0.0} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
  \end{tabular}
  \label{tab:quant_stat}
\end{table*}


\section{Hyperparemeter tuning for CAT}\label{sec:hyperparam}
Since no ground truth exists for our contrastive explanations, hyperparameters for CAT objective (given in Eq.\ref{eqn:main}) were tuned qualitatively by observation. It is important to consider that, in practice a user will only need to tune the hyperparameters once at the beginning and will then be able to generate explanations for an arbitrary number of instances from the dataset. Our tuning led to the following values which we used across datasets: We kept highest weights for $\lambda = 5.0$ to make sure that perturbed sentences have a label different from that of original sentence. We used mean of BERT logits of words inserted/replaced as a surrogate for $p_{LM}(x')$ with regularization parameter $\eta$ set to be $1.0$ and regularization parameter $\nu$ for Levenshtein distance set to $2.0$. $\beta$ was set to $3.0$. The threshold for predicting addition or removal of attributes $\tau$, we used two values. For binary attribute classifiers from the Huffpost News dataset, we set $\tau = 0.3$, and for multiclass attribute classifiers trained on the 20 Newsgroup dataset, we set $\tau=0.05$.

We took 50 randomly selected examples from the training set, generated explanations and evaluated them manually to choose hyperparameters which is similar to prior works \cite{CEM-MAF, gyc}. The boundary values for hyperparameter search were $\lambda \in [4,10]$, $\beta \in [1,5]$, $\eta \in [0.5, 2]$, $\nu \in [1,4]$, and $\tau \in [0.01, 0.5]$.
With more examples for tuning we would expect better explanations, although we found this number to be sufficient.

\section{Attribute classifiers}\label{sec:attr}
In our experiments we created 42 attributes from Huffpost News-Category dataset\cite{news_category} and 20 Newsgroups \cite{kaggle20NewsGrp}.

News-Category dataset \footnote{\url{https://www.kaggle.com/rmisra/news-category-dataset}} has 41 classes of which we merged similar classes and removed those which weren't standard topic. For instance, classes ``\textit{food \& drink}" and ``\textit{taste}" was merged and labelled as a new class ``\textit{food}". At the end we obtained the following 22 classes: \textit{education, money, world, home \& living, comedy, food, black voices, parenting, travel, sports, women, religion, Latino voices, weddings, entertainment, crime, queer voices, arts, politics, science, fifty}, and \textit{environment}. We created 22 1-vs-all binary classifiers, so that the same sentence can have multiple classes. To alleviate the class imbalance issue in training these binary classifiers we sampled fewer instances uniformly at random from the negative classes making sure that the number of negative instances are no more than $80\%$ of the training data.

The 20 Newsgroup dataset \footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.fetch_20newsgroups.html}} has the following 20 classes: \textit{atheism, graphics, ms-windows.misc, computer, mac.hardware, ms-windows.x, forsale, autos, motorcycles, baseball, hockey, cryptography, electronics, medicine, space, christian, guns, mideast, politics}, and \textit{religion}. A distilbert multi-class classifier was trained on this data.

All attribute classifiers were trained with DistliBERT base \footnote{\url{https://huggingface.co/distilbert-base-uncased}} for $10$ epochs using the Adam optimizer with a learning rate of $5\times 10^{-5}$, weight decay of $0.01$, and a batch size of $16$. Each of the models were trained using NVIDIA V100 GPUs in under 12 hours.

\section{Text classifiers}\label{sec:classifier_details}
We conducted experiments on two sets of text classifiers trained on four datasets: One set to compare CAT with GYC and another to compared CAT with MICE. All experiments were run on NVIDIA V100 GPUs.

For experiments comparing CAT with GYC\cite{gyc}, we trained model with the same architecture as the one used in their paper. This model is composed of an \textit{EmbeddingBag} layer followed by a linear layer, a \textit{ReLU} and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss. A GPT2 tokenizer \footnote{\url{https://huggingface.co/gpt2-medium}} was used to convert text into bag of words. The models were trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$.

For experiments comparing CAT with MICE\cite{mice}, we used author provided implementation\footnote{\url{https://github.com/allenai/mice}} to train models with \texttt{AllenNLP} \cite{allennlp}. This architecture is composed of a \textit{RoBERTa-base} model with a linear layer. For all four datasets the models were trained for $5$ epochs with batch size of $8$ using Adam optimizer with a learning rate of $4e-05$, weight decay of $0.1$, and slanted triangular learning rate scheduler with cut frac $0.06$.

\section{Datasets}\label{sec:datasets}
We performed experiments on 4 datasets: AgNews\cite{AgNews2015}, NLI\cite{nli}, DBpedia \cite{Lehmann2015DBpediaA}, and Yelp\cite{Shen2017}. AgNews dataset was taken from Kaggle website \footnote{\url{https://www.kaggle.com/datasets/amananandrai/ag-news-classification-dataset}} and rest three datasets from \textit{huggingface datasets}\cite{hf_datasets}.

\textbf {AgNews}. The dataset is from a real-world news domain which contains short news headlines and bodies from four new categories - world, business, sports, and sci-tech. It contains ~30K training and ~1.9K test examples per class, comprising of ~128K samples. Our experiments focus on explanations for predicting the class from the headlines.

\textbf{NLI}. The Natural Language Inference \cite{nli} dataset\footnote{\url{https://huggingface.co/datasets/snli}} contains samples of two short ordered texts, and the labels are either \textit{contradiction} if the second text contradicts the first, \textit{neutral} if the two texts do not contradict or imply one another, or \textit{entailment} if the second text is a logical consequence of the first text. The dataset contains ~550K training, 10K test and 10K validation examples.

\textbf{DBpedia}. This dataset is a subset of original DBpedia data which is a crowd-sourced community effort to extract structured information from Wikipedia. This dataset\footnote{\url{https://huggingface.co/datasets/dbpedia_14}} is constructed by picking 14 non-overlapping classes from DBpedia 2014 with 40K training and 5K test examples per class. Task here is to predict the class a DBpedia entry belong to. In our experiments we only use \textit{content} and drop the \textit{title} field provided with with the dataset.

\textbf{Yelp}. This is a binary sentiment classification dataset\footnote{\url{https://huggingface.co/datasets/yelp_polarity}} containing 560K highly polar reviews for training and 38K for testing. The dataset consists of reviews from Yelp which is extracted from the Yelp Dataset Challenge 2015.


\section{Quantitative Evaluation Statistics}\label{sec:quant_stat}
Table \ref{tab:quant} (in the main paper) shows the performance evaluation of our proposed approach, CAT, on five different datasets and $2$ classifier models, namely Embedding Bag based classifier and Roberta based classifier models. It was noted that CAT outperformed GYC  and MICE over AgNews, Yelp and Dbpedia by statistically significant margins on respective model. Recall that GYC usage Embedding Bag based classifier model and MICE usage Roberta based classifier. Therefore, we implemented both the classifier models with CAT to compare both GYC and MICE.  We verify this statement in Table \ref{tab:quant_stat} where we report pairwise t-tests comparing the means for CAT with GYC and CAT with MICE and standard deviation of CAT, GYC, MICE for each metric and dataset.  The improvement of CAT over GYC and MICE is observed to be statistically significant across all metrics. We do not report additional statistics for the flip rate metric as CAT always produces a contrastive sentence with a flipped class label unlike GYC or MICE which sometimes fails to flip.

% \section{Additional Setup Details}
% All experiments were run on NVIDIA V100 GPUs. Of the four data sets experimented in the paper, models trained on NLI \eat{and the Hate Speech dataset} were directly taken from the huggingface website\footnote{\url{https://huggingface.co/roberta-large-mnli} \eat{\\\url{https://huggingface.co/cardiffnlp/twitter-roberta-base-hate}}}. %Yelp, AgNews, and DBpedia were trained 
% %\textcolor{blue}{Amar to add details of BoW models such as architecture, optimizer, learning rate etc.}
% The black box models for AgNews, DBPedia and Yelp is composed of an \textit{EmbeddingBag} layer followed by a linear layer, a \textit{ReLU} and another linear layer to obtain the logit. The logit is provided to a classifier we trained with cross entropy loss for 4, 14 and 2 classes for AgNews, DBPedia and Yelp, respectively. A GPT2 tokenizer \footnote{\url{https://huggingface.co/gpt2-medium}} was used to convert text into bag of words. We choose this model architecture to match the models used in GYC \cite{gyc}. The model is trained using the Adam optimizer with a learning rate of $1\times 10^{-3}$, weight decay of $0.01$, and a batch size of $32$. Our code is licensed under Apache-2.0.

\section{Additional Information for User Study}
Figure \ref{fig:userinstr} shows screenshots of user study 1, including the instructions and example questions for the three different methods discussed in the study. The same instructions and format was used for user study 2, except that we asked five task oriented questions (rather than seven) per explainer as there were four explainers (as opposed to 3) keeping the total number of questions to be 24, and thus keeping the overall effort of both user studies roughly the same for participants. For the users the methods were named as Explainer A, B and C, where they correspond to GYC, CAT, and CAT-na respectively for user study 1. For user study 2, Explainer A, B, C and D corresponded to MICE, MICE-nft, CAT and CAT-na. Some users also left optional comments at the end of the user study which we list here:

\begin{itemize}
    \item ``I found the questions confusing... What is complete, sufficient and understandable explanation in a word change? Also, in each example, what was I supposed to guess, the category of the article or the possible prediction of the method? Are those things different?'' (Study 1)
    \item ``Explainer A was pretty bad, explainer B was very good, and explainer C was reasonably good.'' (Study 1)
    \item ``Explainer b was the best. The q\&a at the end of each page allows multiple choices per row, which is bad. Each question should remove the modified classification as an option (if the modified sentence is World, I shouldn't be allowed to choose World). Early on the survey should state clearly that there are only 4 categories (business/sci-tech/sports/world) which I didn't know right away, I expected each question have 4 different options, and knowing this might have helped me understand what we're doing here better. The opening text was very confusing.'' (Study 1)
    \item ``I found B to be the best one.'' (Study 1)
    \item ``nice survey'' (Study 1)
    \item ``the additional info in explanation C was useful'' (Study 2)
\end{itemize}



\begin{figure*}[htbp]
\centering
 \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/CAT_instr.png}
        \caption{}
    \end{subfigure}
     \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/likert_ss.png}
        \caption{}
    \end{subfigure}\\
   %\vspace{0.2cm}
   \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/gyc_ss.png}
        \caption{}
    \end{subfigure}
   \hspace{0.1\textwidth}
   \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/cat_ss.png}
        \caption{}
    \end{subfigure}
  \caption{In (a) we show the instructions for the survey. In (b) we see the qualitative questions. In (c) and (d) we see the task oriented questions for GYC and CAT respectively.} 
\label{fig:userinstr}
%\vspace{-0.3cm}
\end{figure*}

\section{Additional Qualitative Examples}\label{sec:qualitative_examples}
Table \ref{tab:extra_examples} offers at least five more examples of contrastive explanations from each dataset. Additional insight can be gained from the attributes; in the first row, adding travel-related text can flip the class from business to world, i.e., the article was predicted business because if it was more about travel it would have been predicted as world. This type of explanation adds extra intuition as opposed to only being given the replacement of words, ``oil" to ``winds" in this case. As can also been seen, insight is also a function of using attributes that have a relationship to the dataset and task. For example, attributes derived from news sources are often not helpful for explaining sentiment classifiers (e.g., Yelp) for which sentiment is often flipped by the negation of the text. This is to be expected; good explanations require good attributes.

\begin{table*}[htbp]
\centering
\small
\caption{Extra contrastive explanation examples from four datasets: AgNews, NLI, DBPedia, and Yelp.}
\label{tab:extra_examples}
% \begin{tabular}{|p{7cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\begin{tabular}{|p{5.75cm}|p{4cm}|p{3cm}|p{3cm}|p{1cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Input/CAT}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Attribute Changes}}}  & \multicolumn{1}{c|}{\textbf{Input}} & \multicolumn{1}{c|}{\textbf{Contrast}}
& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}}\\
   &  & \multicolumn{1}{c|}{\textbf{Pred}}  &\multicolumn{1}{c|}{\textbf{Pred}}&  \\ \hline

\st{Oil} \textcolor{red}{Winds} Up from 7-Week Lows on U.S. Weather & \multicolumn{1}{c|}{+travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{world} & AgNews \\ \hline

New Hummer Is Smaller, Cheaper and Less \st{Gas} \textcolor{red}{cpu} Hungry & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -travel, \\-space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ 
\hline

Perfect start for France in \st{Federation} \textcolor{red}{Microsoft} Cup & \multirow{2}{*}{\shortstack{+cryptography, -motorcycles, \\-hockey, -space, -politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\ \hline
%\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey}& \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\st{Kuwait} \textcolor{red}{Source}: Fundamentalists Recruiting Teens (AP) &  \multicolumn{1}{c|}{+guns, religion, -mideast}& \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} & AgNews \\ \hline

\multirow{2}{*}{Harry \st{in nightclub} \textcolor{red}{inflight} scuffle}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+sports, +space, -religion, \\-cryptography, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{AgNews}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline
\eat{
I thought you \textcolor{red}{ladies} were leaving the country you washed up \$\$\$\$ \$\$\$\$? & \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -cryptography}}& \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

Such crimes must attract severest punishment,say Min Jail term of 25Y. If they r \st{illegal} \st{migrants} \textcolor{red}{convicted}, force them to leave the Country immediately& \multicolumn{1}{c|}{\multirow{3}{*}{+atheism, -politics}} & \multicolumn{1}{c|}{\multirow{3}{*}{hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{3}{*}{Hate}} \\ \hline

\multirow{2}{*}{\st{@brianstelter} \textcolor{red}{she} is a complete \st{joke} \textcolor{red}{\$\$\$\$} ! if you see...}& 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +cryptography, \\-sports, -politics}} }& \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

Do \st{you} \textcolor{red}{chicks} ever \st{rap} \textcolor{red}{talk} in your whitest voice possible or is that just me?& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+parenting, +atheism, +politics \\-world, -sports, -arts}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline

\st{There's} \textcolor{red}{Women} \textcolor{red}{get} no greater satisfaction than knowing you did it yourself' -me when someone asks me ... & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+women, +entertainment, \\ +religion, -sports}}} & \multicolumn{1}{c|}{\multirow{2}{*}{not hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{hate}} & \multicolumn{1}{c|}{\multirow{2}{*}{Hate}} \\ \hline
}
Five soldiers hold and aim their \st{weapons} \textcolor{red}{blades}. $<$/s$>$ The soldiers are \st{eating} \textcolor{red}{armed}.
& \multicolumn{1}{c|}{\multirow{2}{*}{-guns}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Skateboarder jumps of off dumpster. $<$/s$>$ a \st{bike} \textcolor{red}{young} rider in a race&
 \multicolumn{1}{c|}{\multirow{2}{*}{+world}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

Two people walking down a dirt trail with backpacks on looking at \st{items} \textcolor{red}{map} they are carrying. $<$/s$>$ One is holding a map.
& \multicolumn{1}{c|}{\multirow{3}{*}{+space, -motorcyles, -electronics}}& \multicolumn{1}{c|}{\multirow{3}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

A brown and black dog is jumping to catch a red ball. $<$/s$>$ Two dogs are
\textcolor{red}{not} playing catch with their owner.
& \multicolumn{1}{c|}{\multirow{2}{*}{-arts}}& \multicolumn{1}{c|}{\multirow{2}{*}{neutral}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{NLI}} \\  \hline

A girl is standing in a field pushing up her hat with one finger and her hand is
covering most of her face. $<$/s$>$ A \st{girl} \textcolor{red}{boy} covers her face. 
& \multicolumn{1}{c|}{\multirow{3}{*}{+parenting, -medicine}}& \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{entail\\-ment}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{contra\\-diction}}} & \multicolumn{1}{c|}{\multirow{3}{*}{NLI}} \\  \hline

Channel Chaos is a 1985 Australian \st{film} \textcolor{red}{production} set at a TV station & \multicolumn{1}{c|}{\multirow{2}{*}{+electronics, -travel, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{film}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

\multirow{2}{*}{Dinik is a \st{village} \textcolor{red}{lake} in Croatia}
& \multicolumn{1}{c|}{\multirow{2}{*}{+medicine, +space, -mideast}}& \multicolumn{1}{c|}{\multirow{2}{*}{village}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{natural\\place}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

%\multirow{2}{*}{Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}}
Air Cargo Mongolia is a Mongolian \st{airline} \textcolor{red}{newspaper}
& \multicolumn{1}{c|}{\multirow{2}{*}{+politics, -space}}& \multicolumn{1}{c|}{\multirow{2}{*}{plant}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{written\\work}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ 
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

ACTION is a bus service \st{operator} \textcolor{red}{based} in Canberra Australia
& \multicolumn{1}{c|}{\multirow{2}{*}{+autos, -electronics}}& \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{transport\\-ation}}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

Jagjaguwar is an indie rock record \st{label} \textcolor{red}{musician} based in Bloomington Indiana 
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+space, +politics, -world \\-forsale, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{company}} & \multicolumn{1}{c|}{\multirow{2}{*}{artist}} & \multicolumn{1}{c|}{\multirow{2}{*}{DBPedia}} \\ \hline

he \st{really} \textcolor{red}{hardly} made our anniversary dinner entertaining memorable
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +sports, +cryptography \\-home\&living, -electronics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

they also have deep fried desserts if you're \st{brave} \textcolor{red}{poor} enough
& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+medicine, -travel \\-religion, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\ \hline

i \st{definitely} \textcolor{red}{never} will go back & \multicolumn{1}{|c|}{-entertainment} &\multicolumn{1}{c|}{positive}&\multicolumn{1}{c|}{negative}&\multicolumn{1}{c|}{Yelp} \\ \hline

\multirow{2}{*}{jesse is completely \st{rude} \textcolor{red}{perfect}}& \multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+cryptography, -entertainment, \\-medicine, -space}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline

\multirow{2}{*}{the pizza \st{sauce} \textcolor{red}{heaven} is also way too sweet} & 
\multicolumn{1}{c|}{\multirow{2}{*}{\shortstack{+world, +travel, +arts, +atheism \\+religion, -medicine, -politics}}} & \multicolumn{1}{c|}{\multirow{2}{*}{negative}} & \multicolumn{1}{c|}{\multirow{2}{*}{positive}} & \multicolumn{1}{c|}{\multirow{2}{*}{Yelp}} \\
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}\\ \hline


\eat{
\multirow{2}{*}{Kazaa Owner Cheers \st{File} \textcolor{red}{Salary}-Swapping Decision (AP)} \quad\quad\quad\quad\quad\quad\quad\quad & \multirow{2}{*}{\shortstack{+forsale, +baseball, +hockey,\\ -arts, -windows, -cryptography}} & \multicolumn{1}{c|}{\multirow{2}{*}{sci-tech}} & \multicolumn{1}{c|}{\multirow{2}{*}{sports}} & \\
\hline

New Human Species \st{Discovered} \textcolor{red}{influenza} & +medicine, -cryptography & \multicolumn{1}{c|}{sci-tech} & \multicolumn{1}{c|}{world} \\ \hline

US shows flexibility on \st{Israeli} \textcolor{red}{virtual} settlements & +arts, +cryptography, -mideast & \multicolumn{1}{c|}{world} & \multicolumn{1}{c|}{sci-tech} \\ \hline


\eat{Will sinking Lowe resurface in \st{playoffs} \textcolor{red}{2020}? & \multicolumn{1}{c|}{+space, -hockey} & \multicolumn{1}{c|}{sports} & \multicolumn{1}{c|}{business} \\ \hline}

Pace of U.S. \st{Factory} \textcolor{red}{population} Growth Climbs in Dec & \multicolumn{1}{c|}{+politics, -money, -travel} & \multicolumn{1}{c|}{business} & \multicolumn{1}{c|}{sci-tech} \\ \hline

It may take 146 years for Nigeria to wipe out \st{corruption} \textcolor{red}{funds} from \st{its} \textcolor{red}{bank} system going by the latest report ...\eat{by Transparency International (TI) which gave the country the third position among the most corrupt countries of the world} & \multicolumn{1}{c|}{\multirow{2}{*}{+ money, - politics}} & \multicolumn{1}{c|}{\multirow{2}{*}{world}} & \multicolumn{1}{c|}{\multirow{2}{*}{business}} \\ \hline
}
\end{tabular}
 \end{table*}
 
%\section{Limitations}
%Since our explanation is based on BERT which is pretrained for natural languages, it might have difficulties with informal or non grammatical sentences such as those coming from tweets. However, the limilation  can be potentially alleviated by language model fine tuning on the relevant dataset, e.g. on a tweet dataset, or by using other language models that are tailored to specific use cases.


% Since our explanation is based on natural language model (BERT), it might have difficulties with informal or non grammatical sentences such as those coming from tweets. The reason is due to a dependency on BERT, but if issues arise, this could potentially be fixed with other language models that are tailored to specific usecases.

\eat{The main limitation to our CAT method is the need for attribute classifiers. However, as noted in the paper, the attributes can be derived from other sources of data and not necessarily be dependent on the data and model being explained. Furthermore, there are other methods to obtain attributes. Unsupervised methods such as LDA, VAEs, GANs could be leveraged to ascertain semantically meaningful attributes. The attribute classifier that appears in our loss function could be replaced by disentangled representations learned by VAEs \cite{DIP-VAE} or by topic models. This shows that CAT is not limited to only annotated datasets.} 







% \begin{table*}[!]
%  \centering
% \caption{We evaluate CAT on three metrics:  i) \textbf{Dist}(distance), ii) \textbf{Fluency}, iii) \textbf{Cont} (content preservation).  We report p-values from a pairwise t-test of the difference of means between GYC and CAT for all metrics. As can be seen by the negligible p-values, CAT is (statistically) significantly better than GYC. We also report standard deviation (std. dev.) for all metrics for CAT and GYC, which together with the means reported in the main paper, are used to run the t-tests.
% }
%  \label{tab:quant_stat}
% \begin{tabular}{l|ccc|ccc}
% \multicolumn{7}{c}{}\\
% \multirow{3}{*}{Stat} &
%      \multicolumn{3}{c|}{AgNews} &
%       \multicolumn{3}{c}{Yelp} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%       & Dist & Cont & Fluency &
%       Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%     %   GYC & \multicolumn{4}{c|}{NR} & \multicolumn{4}{c}{NR}\\
%       p-value   &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$   &$< 1e^{-8}$  &$< 1e^{-8}$  &$< 1e^{-8}$  \\
%       \midrule
%       std. dev. (MICE)   &0.182   &0.121   &0.196  &0.174  &0.109  &0.208  \\
%       std. dev. (MICE-nft)   &0.307   &0.209   &0.224  &0.240  &0.154  &0.212  \\
%       std. dev. (CAT)   &0.307  &0.209 &0.144  &0.0 &0.0 &0  \\
      
%     %   std. dev. (CAT-na)   &\textbf{0.101}  &\textbf{0.072}  &\textbf{0.145} &\textbf{0.0} &\textbf{0.0} &\textbf{0.0}  \\
%       \bottomrule
%   \end{tabular}
  
%  \begin{tabular}{l|cccccccc}
% \multicolumn{4}{c}{}\\
% \multirow{3}{*}{Stat} &
%     %  \multicolumn{4}{c|}{NLI} &
%       \multicolumn{3}{c}{Dbpedia} \\
%       %& $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\approx 1$ \\
%     %   & Flip & Dist & Cont & Fluency 
%       & Dist & Cont & Fluency\\
% %       \cmidrule{1-9}
%         \midrule
%       p-value  &$< 1e^{-8}$  &$< 1e^{-8}$  & $< 1e^{-8}$ \\
%       \midrule
%       std. dev.(MICE)  &0.151   &0.077   &0.168 \\
%       std. dev.(MICE-nft)  &0.200  &0.160  &0.160 \\
%       std. dev.(CAT)   &0.0  &0.0  &0.0 \\
      
%     %   std. dev.(CAT-na)   &\textbf{0.0}  &\textbf{0.0}  &\textbf{0.0} \\
%     %   &\textbf{1} &\textbf{0.07} &\textbf{0.97} &\textbf{1.02} \\
%       \bottomrule
%   \end{tabular}
  
% % \begin{tabular}{l|cccccccc}
% % \multicolumn{4}{c}{}\\
% % \multirow{3}{*}{Method} &
% %       \multicolumn{4}{c}{Hate Speech} \\
% %       & Flip & Dist & Cont & Fluency\\
% %         \midrule
% %       CAT &\textbf{1} &\textbf{0.08} &\textbf{0.98} & \textbf{1.03}\\
% %       \bottomrule
% %   \end{tabular}
%   \label{tab:quant_stat}
% \end{table*}


==> userstudy.tex <==
We now describe a user study we conducted to ascertain the value of our attributed explanations. User studies having become ubiquitous in explainable AI literature \cite{lime, acd, mame, CEM-MAF} because they illustrate the benefit of these tools to the end user. We follow in the direction of most user studies by ascertaining benefit by requiring participants to perform a task  given our explanations, as opposed to solely asking users the utility of our method.

\noindent\textbf{Methods:} We consider three different explanation methods: 1) CAT, 2) CAT-na (i.e. CAT without attributes) and 3) GYC. Comparison of CAT with CAT-na provides an ablation, while its comparison with GYC showcases its value relative to other state-of-the-art contrastive text explanations.

\noindent\textbf{Setup:} The AgNews dataset was used for the study. We built a four class neural network black box model (described earlier) to predict articles as either belonging to Business, Sci-Tech, World or Sports categories. The task given to users was to determine the classification of the article based on a contrastive explanation from one of the respective methods. Five options were provided to the user which included the four classes along with a ``Can't Tell" option. For each method, seven randomly chosen sentence-explanation pairs were provided to the user where the users were blinded to the exact method producing the explanation. For each (anonymized) explanation method, we additionally asked the users for their qualitative assessment along four dimensions; completeness, sufficiency, satisfaction and understandability based on a 5 point Likert scale. Thus, there were a total of 24 questions that users answered. Users were also allowed to leave optional comments which we provide in the Supplement, along with screen shots from the user study. %Predicting black box outputs or simulatibility is a standard procedure to measure the efficacy of explanations \cite{mame,lime,lipton2016mythos}.

We hosted our survey on Google Forms. 37 participants from quantitative backgrounds including data science, engineering and business analytics took part in the study. We did this as recent work shows that most consumers of such explanations have these backgrounds \cite{umang}.


\noindent\textbf{Observations:} 
Figure \ref{fig:userstudy} depicts the results from our user study. The top figure demonstrates that both our methods CAT and its ablation CAT-na (which does not use attributes) significantly outperform GYC in terms of usability towards the task. Moreover, the benefit of the attributes is also evident as CAT not only does better than CAT-na in terms of ``Correct" responses, but it also has fewer ``Wrong" answers with some of this gap being attributed to ``Cannot Tell". This indicates that the insight CAT provides through attributes helps users err on the side of caution, rather than convincing them of something that is incorrect.

Our method performs much better than GYC and the ablation from a qualitative perspective, as well, as seen in Figure \ref{fig:userstudy} (bottom). These qualitative preferences of CAT are further confirmed through the (optional) comments written by some participants, e.g., ``... explainer B was very good, and explainer C was reasonably good", where ``explainer B" refers to CAT and ``explainer C" to CAT-na. %An exhaustive list of comments is provided in the Supplement, along with screen shots of the survey.



